A Comprehensive Survey of Machine Learning Based Localization with Wireless Signals

The last few decades have witnessed a growing interest in location-based services. Using localization systems based on Radio Frequency (RF) signals has proven its efficacy for both indoor and outdoor applications. However, challenges remain with respect to both complexity and accuracy of such systems. Machine Learning (ML) is one of the most promising methods for mitigating these problems, as ML (especially deep learning) offers powerful practical data-driven tools that can be integrated into localization systems. In this paper, we provide a comprehensive survey of ML-based localization solutions that use RF signals. The survey spans different aspects, ranging from the system architectures, to the input features, the ML methods, and the datasets. A main point of the paper is the interaction between the domain knowledge arising from the physics of localization systems, and the various ML approaches. Besides the ML methods, the utilized input features play a major role in shaping the localization solution; we present a detailed discussion of the different features and what could influence them, be it the underlying wireless technology or standards or the preprocessing techniques. A detailed discussion is dedicated to the different ML methods that have been applied to localization problems, discussing the underlying problem and the solution structure. Furthermore, we summarize the different ways the datasets were acquired, and then list the publicly available ones. Overall, the survey categorizes and partly summarizes insights from almost 400 papers in this field. This survey is self-contained, as we provide a concise review of the main ML and wireless propagation concepts, which shall help the researchers in either field navigate through the surveyed solutions, and suggested open problems.

==> Abstract.tex <==





A main point of the paper is the interaction between the domain knowledge arising from the physics of localization systems, and the various ML approaches. Besides the ML methods, the utilized input features play a major role in shaping the localization solution; we present a detailed discussion of the different features and what could influence them, be it the underlying wireless technology or standards or the preprocessing techniques. Furthermore, we summarize the different ways the datasets were acquired and whether they are  publicly available. A key part of the paper is then the summary of which ML methods have been applied to which localization problems, categorizing and partly summarizing the insights from almost 400 papers in this field.  
This survey is self-contained, as we provide a concise review of the main ML and wireless propagation concepts, which shall help the researchers in either field navigate through the surveyed solutions,  and  suggested open problems.

==> AllTables/DataSourceTbl.tex <==
\begin{tabularx}{\textwidth} { 
  | >{\raggedright\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.5\hsize}X 
  | >{\centering\arraybackslash\hsize=.5\hsize}X |}
 \caption{Test data}
 \hline
  & Measurement & Simulation & Ray tracing & Open Dataset \\
 \hline
 Code unavailable online & ~\cite{alteredAP} ~\cite{MLthesis} ~\cite{8651736} ~\cite{7743685} ~\cite{MonoDCell} ~\cite{vlfANN} ~\cite{7938617} ~\cite{OnDevice} ~\cite{lorawan} ~\cite{telco} ~\cite{6805641} ~\cite{wsn_svr} ~\cite{RadioMaps} ~\cite{tlfcma} ~\cite{LowOverhead} ~\cite{magnetic_inertial} ~\cite{IndustrialWSN} ~\cite{uav} ~\cite{location_aware} ~\cite{8240410} ~\cite{8108573} ~\cite{OpticalCamera} ~\cite{devicefree} ~\cite{IndoorOutdoor} ~\cite{10.1145/3321408.3321584} ~\cite{8780770} ~\cite{8673800} ~\cite{pseudolite} ~\cite{rfid} ~\cite{kmgpr} ~\cite{8765368} ~\cite{Discriminative} ~\cite{DataAugmentation} ~\cite{8362712} ~\cite{Eloc} ~\cite{HumanDetection} ~\cite{RelationLearning} ~\cite{FullBandGSM} ~\cite{grof} ~\cite{hapi} ~\cite{mmbp} ~\cite{hiwl} ~\cite{7064997} ~\cite{WeightedAmbientWiFi} ~\cite{eee112} ~\cite{8008794} ~\cite{8584443} ~\cite{8543713} ~\cite{JUIndoorLoc} ~\cite{7313038} ~\cite{8931646} ~\cite{LiUnsupervised} ~\cite{yang2012locating} ~\cite{8115921} ~\cite{8661625} ~\cite{Wang2017WiFiFB} ~\cite{Chunjing2017WLAN} ~\cite{8422182} ~\cite{wu2019mobile} ~\cite{feng2019received} ~\cite{zhang2017efficient} ~\cite{xu2019efficient} ~\cite{cottone2016machine} ~\cite{pelka2018new} \cite{sun2008adaptive} \cite{cheng2018fingerprint} ~\cite{khatab2017fingerprint} ~\cite{yan2018noise} ~\cite{wang2019robust} ~\cite{mei2018novel} ~\cite{wu2018accurate} ~\cite{nguyen2017performance} ~\cite{musa2019decision} ~\cite{zou2015fast} ~\cite{rezgui2017efficient} ~\cite{figuera2012advanced} ~\cite{guo2018accurate} ~\cite{bi2018adaptive} ~\cite{elbes2019indoor} ~\cite{comiter2018localization} ~\cite{liu2019hybrid} ~\cite{liu2017wicount} ~\cite{ahmadi2017exploiting} ~\cite{adege2018indoor} ~\cite{adege2019mobility} ~\cite{schmidt2019sdr} ~\cite{gu2015online} ~\cite{yang2018clustering} ~\cite{yan2017hybrid} ~\cite{malik2019indoor} ~\cite{bae2019large} ~\cite{wang2019indoor} ~\cite{tewes2019ensemble} ~\cite{sung2019neural} ~\cite{li2017measurement} ~\cite{zhou2019smartphone} ~\cite{sanam2018improved} ~\cite{xiao2012large} ~\cite{zhao2019accurate} ~\cite{salamah2016enhanced} ~\cite{widmaier2019towards} ~\cite{homayounvala2019novel} ~\cite{savic2014kernel} ~\cite{zhang2019improving} ~\cite{belmonte2019swiblux} ~\cite{li2019smartloc} ~\cite{dashti2016extracting} ~\cite{livinsa2015localization} ~\cite{yang2012locating} ~\cite{oussar2011indoor} ~\cite{chen2019dpr} ~\cite{mahfouz2015kernel} ~\cite{qiu2018walk} ~\cite{yan2015improved} & ~\cite{FPfusing} ~\cite{InterpretingCNN} ~\cite{MLthesis} ~\cite{MassiveMIMO} ~\cite{7504333} ~\cite{msvr} ~\cite{NLOS_UWB} ~\cite{6488858} ~\cite{sdr} ~\cite{TargetTracking} ~\cite{tdoa} ~\cite{patent} ~\cite{manifold} ~\cite{FineGrainedSubcarrier} ~\cite{ZhangIndoor} ~\cite{8712551} ~\cite{AntonioLocalization} ~\cite{7996460} ~\cite{jaafar2018neural} ~\cite{ge2019hybrid} \cite{felix2016fingerprinting} ~\cite{comiter2017data} ~\cite{comiter2017structured} ~\cite{zou2015fast} ~\cite{afzal2014localization} ~\cite{lee2013new} ~\cite{wang2007agent} ~\cite{comiter2018localization} ~\cite{zhang2018heterogeneous} ~\cite{yi2019neural} ~\cite{bhatti2018machine} ~\cite{tran2008localization} ~\cite{feng2010location} ~\cite{xiao2018learning} ~\cite{mahfouz2015kernel} ~\cite{yan2015improved} & ~\cite{mmwave} ~\cite{AntonioLocalization} & ~\cite{mmwave} ~\cite{gbrbm} ~\cite{kmgpr} ~\cite{Timotheatos2017FeatureEA} ~\cite{FeatureSelection} ~\cite{hybloc} ~\cite{Qian2019Supervised} ~\cite{wang2019robust} ~\cite{nguyen2017performance} ~\cite{al2018improved} ~\cite{zhang2018enhancement} ~\cite{tewes2019ensemble} ~\cite{kim2018hybrid} ~\cite{xiao2018learning} ~\cite{patel2020millimeter}\\
 \hline
 Code available online &  &  &  & ~\cite{csiRNN} ~\cite{kim2018scalable} ~\cite{secckin2019hierarchical}\\
 \hline
\end{tabularx}


==> AllTables/DataSourceTbl2.tex <==
\begin{tabularx}{\textwidth} { 
  | >{\raggedright\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.5\hsize}X 
  | >{\centering\arraybackslash\hsize=.5\hsize}X |}
 \caption{Test data}
 \label{tab:Dataset}
 \hline
  & Measurement & Simulation & Ray tracing & Open Dataset \\
 \hline
 Code unavailable online & ~\cite{alteredAP,MLthesis,8651736,7743685,MonoDCell,vlfANN,7938617,OnDevice,lorawan,telco,6805641,wsn_svr,RadioMaps,tlfcma,LowOverhead,magnetic_inertial,IndustrialWSN,uav,location_aware,8240410,8108573,OpticalCamera,devicefree,10.1145/3321408.3321584,8780770,8673800,rfid,kmgpr,8765368,Discriminative,DataAugmentation,8362712,Eloc,HumanDetection,RelationLearning,FullBandGSM,grof,hapi,mmbp,hiwl,7064997,WeightedAmbientWiFi,eee112,8008794,8584443,JUIndoorLoc,7313038,8931646,LiUnsupervised,yang2012locating,8115921,8661625,Wang2017WiFiFB,Chunjing2017WLAN,8422182,wu2019mobile,feng2019received,zhang2017efficient,xu2019efficient,cottone2016machine} \cite{sun2008adaptive} \cite{cheng2018fingerprint,khatab2017fingerprint,yan2018noise,wang2019robust,mei2018novel,wu2018accurate,nguyen2017performance,musa2019decision,zou2015fast,rezgui2017efficient,figuera2012advanced,guo2018accurate,bi2018adaptive,elbes2019indoor,comiter2018localization,liu2019hybrid,liu2017wicount,ahmadi2017exploiting,adege2018indoor,adege2019mobility,schmidt2019sdr,gu2015online,yang2018clustering,yan2017hybrid,malik2019indoor,bae2019large,tewes2019ensemble,sung2019neural,li2017measurement,sanam2018improved,xiao2012large,zhao2019accurate,salamah2016enhanced,widmaier2019towards,homayounvala2019novel,zhang2019improving,belmonte2019swiblux,li2019smartloc,dashti2016extracting,yang2012locating,oussar2011indoor,chen2019dpr,mahfouz2015kernel,qiu2018walk,van2015machine_1,niitsoo2019deep_2,wang2016csi_3,wang2016csi_5,wu2019csi_7,li2018channel_8,wang2017cifi_9,niitsoo2018convolutional_11,li2019convolutional_12,rizk2018cellindeep_15,aikawa2019cnn_16,wang2018deep_23,hsieh2019deep_28,li2019deep_31,gan2017deep_32,wang2015deepfi_33,yazdanian2018deeppos_34,berruet2018delfin_35,xue2019deeptal_36,zhang2016deep_38,wang2017biloc_43,wu2017passive_44,ghourchian2017real_45,zhou2017robust_46,sorour2014joint_47,zhang2020transfer_49,shokry2018deeploc_50,ouyang2011indoor_51,liu2009low_52,gu2015semi_54,pulkkinen2011semi,zhou2017semi_55,wang2017resloc_56,aikawa2018wlan_61,abbas2019wideep_63,huang2020widet_64,chen2019wifi_65,dayekh2010cooperative,kram2019uwb_68,choi2019unsupervised_69,krishnan2018improving_71,alhajri2019indoor_74,goswami2011wigem_75,zhou2017grassma_76,decurninge2018csi_81,arnold2018deep_82,zhou2017indoor_86,chen2018deep_88,jung2015unsupervised_89,sen2012you_91,wang2012no_92,wu2012will_93,ray2016localization_94,lee2018dnn_95,rizk2019device_96,rizk2019solocell_98,wang2018deepmap_103,liu2018autloc_104,zhang2017deeppositioning_106,tarekegn2019applying_107,zhang2019deeploc_108,mittal2018adapting_109,adege2018applying_113,sobehy2019csi_117,song2019novel_119,shao2018indoor_120,de2019csi_121,choi2019unsupervised_123,own2019signal_125,ebuchi2019vehicle_126,pandey2019handling_127,de2019enhanced_129} & ~\cite{FPfusing,InterpretingCNN,MLthesis,MassiveMIMO,7504333,,NLOS_UWB,sdr,TargetTracking,tdoa,patent,FineGrainedSubcarrier,ZhangIndoor,8712551,AntonioLocalization,jaafar2018neural,ge2019hybrid} \cite{felix2016fingerprinting,comiter2017data,comiter2017structured,zou2015fast,comiter2018localization,zhang2018heterogeneous,yi2019neural,bhatti2018machine,xiao2018learning,mahfouz2015kernel,njima2019deep_22,chen2011semi_53,li2017robust_60,prasad2018machine_62,vieira2017deep_80,prasad2017numerical_84,pirzadeh2019machine_87,sun2018single_90,chen2018multipath_111,xiong2019decorrelation_115,wu2019neural_116,own2019signal_125,lei2019siamese_130} & ~\cite{mmwave,AntonioLocalization,gan2017deep_32,butt2020rf_57,wang2019fast_83,de2019enhanced_129} & ~\cite{mmwave,gbrbm,kmgpr,Timotheatos2017FeatureEA,FeatureSelection,hybloc,Qian2019Supervised,wang2019robust,nguyen2017performance,zhang2018enhancement,tewes2019ensemble,kim2018hybrid,xiao2018learning,patel2020millimeter,qian2019convolutional_10,ibrahim2018cnn_13,turabieh2019cascaded,janssen2019comparing,turgut2019deep_27,wang2020robust_59,ciftler2020federated_70,jang2018indoor_99,nowicki2017low,belmannoubi2019stacked_110,dou2018top_112,song2019novel_119}\\
 \hline
 Code available online &  &  &  & ~\cite{csiRNN,kim2018scalable,secckin2019hierarchical}\\
 \hline
\end{tabularx}

==> AllTables/DataSourceTbl3.tex <==
 
\begin{tabularx}{0.5\textwidth} { 
  | >{\raggedright\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.5\hsize}X 
  | >{\centering\arraybackslash\hsize=.5\hsize}X |}
 \caption{Test data}
  \label{tab:Dataset}
 \hline
  & Measurement & Simulation & Ray tracing & Open Dataset \\
 \hline
 Code unavailable online & ~\cite{alteredAP,8651736,7743685,MonoDCell,vlfANN,7938617,OnDevice,lorawan,telco,6805641,wsn_svr,RadioMaps,tlfcma,LowOverhead,magnetic_inertial,IndustrialWSN,uav,location_aware,8240410,8108573,OpticalCamera,devicefree,10.1145/3321408.3321584,8780770,8673800,rfid,kmgpr,8765368,Discriminative,DataAugmentation,8362712,Eloc,HumanDetection,RelationLearning,FullBandGSM,grof,hapi,mmbp,hiwl,7064997,WeightedAmbientWiFi,eee112,8008794,8584443,JUIndoorLoc,7313038,8931646,LiUnsupervised,yang2012locating,8115921,8661625,Wang2017WiFiFB,Chunjing2017WLAN,8422182,wu2019mobile,feng2019received,zhang2017efficient,xu2019efficient,cottone2016machine, sun2008adaptive,cheng2018fingerprint,khatab2017fingerprint,yan2018noise,wang2019robust,mei2018novel,wu2018accurate,nguyen2017performance,musa2019decision,zou2015fast,rezgui2017efficient,figuera2012advanced,guo2018accurate,bi2018adaptive,elbes2019indoor,comiter2018localization,liu2019hybrid,liu2017wicount,ahmadi2017exploiting,adege2018indoor,adege2019mobility,schmidt2019sdr,gu2015online,yang2018clustering,yan2017hybrid,malik2019indoor,bae2019large,tewes2019ensemble,sung2019neural,li2017measurement,sanam2018improved,xiao2012large,zhao2019accurate,salamah2016enhanced,widmaier2019towards,homayounvala2019novel,zhang2019improving,belmonte2019swiblux,li2019smartloc,dashti2016extracting,yang2012locating,oussar2011indoor,chen2019dpr,mahfouz2015kernel,qiu2018walk,van2015machine_1,niitsoo2019deep_2,wang2016csi_3,wang2016csi_5,wu2019csi_7,li2018channel_8,wang2017cifi_9,niitsoo2018convolutional_11,li2019convolutional_12,rizk2018cellindeep_15,aikawa2019cnn_16,wang2018deep_23,hsieh2019deep_28,li2019deep_31,gan2017deep_32,wang2015deepfi_33,yazdanian2018deeppos_34,berruet2018delfin_35,xue2019deeptal_36} \cite{zhang2016deep_38,wang2017biloc_42} \cite{wu2017passive_44,ghourchian2017real_45} ~\cite{zhou2017robust_46,sorour2014joint_47,zhang2020transfer_49,shokry2018deeploc_50,ouyang2011indoor_51,liu2009low_52,gu2015semi_54,pulkkinen2011semi,zhou2017semi_55,wang2017resloc_56,aikawa2018wlan_61,abbas2019wideep_63,huang2020widet_64 , XYZXYZ, dayekh2010cooperative_66 ,kram2019uwb_68,choi2019unsupervised_69,krishnan2018improving_71,alhajri2019indoor_74,goswami2011wigem_75,zhou2017grassma_76,decurninge2018csi_81,arnold2018deep_82,zhou2017indoor_86,chen2018deep_88,jung2015unsupervised_89,sen2012you_91,wang2012no_92,wu2012will_93,ray2016localization_94,lee2018dnn_95,rizk2019device_96,rizk2019solocell_98,wang2018deepmap_103,liu2018autloc_104,zhang2017deeppositioning_106,tarekegn2019applying_107,zhang2019deeploc_108,mittal2018adapting_109,adege2018applying_113,sobehy2019csi_117,song2019novel_119,shao2018indoor_120,de2019csi_121,choi2019unsupervised_123,own2019signal_125,ebuchi2019vehicle_126,pandey2019handling_127,de2019enhanced_129} 
 
 
 
 & ~\cite{FPfusing,InterpretingCNN,MLthesis,MassiveMIMO,7504333,NLOS_UWB,sdr,TargetTracking,tdoa,patent,FineGrainedSubcarrier,ZhangIndoor,8712551,AntonioLocalization,jaafar2018neural,ge2019hybrid} \cite{felix2016fingerprinting,comiter2017data,comiter2017structured,zou2015fast,comiter2018localization,zhang2018heterogeneous,yi2019neural,bhatti2018machine,xiao2018learning,mahfouz2015kernel,njima2019deep_22,chen2011semi_53,li2017robust_60,prasad2018machine_62,vieira2017deep_80,prasad2017numerical_84,pirzadeh2019machine_87,sun2018single_90,chen2018multipath_111,xiong2019decorrelation_115,wu2019neural_116,own2019signal_125,lei2019siamese_130} & ~\cite{mmwave,AntonioLocalization,gan2017deep_32,butt2020rf_57,wang2019fast_83,de2019enhanced_129} & ~\cite{mmwave,gbrbm,kmgpr,Timotheatos2017FeatureEA,FeatureSelection,hybloc,Qian2019Supervised,wang2019robust,nguyen2017performance,zhang2018enhancement,tewes2019ensemble,kim2018hybrid,xiao2018learning,patel2020millimeter,qian2019convolutional_10,ibrahim2018cnn_13,turgut2019deep_27,wang2020robust_59,ciftler2020federated_70,jang2018indoor_99,nowicki2017low,belmannoubi2019stacked_110,dou2018top_112,song2019novel_119}\\
 \hline
 Code available online &  &  &  & ~\cite{csiRNN,kim2018scalable,secckin2019hierarchical}\\
 \hline
\end{tabularx}
 

==> AllTables/DataSourceTbl4.tex <==
\begin{table}
\begin{tiny}
\begin{scriptsize}
\begin{tabularx}{0.45\textwidth} { 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash\hsize=1.05\hsize}X 
  | >{\centering\arraybackslash\hsize=1.1\hsize}X 
  | >{\centering\arraybackslash\hsize=0.8\hsize}X 
  | >{\centering\arraybackslash\hsize=1.1\hsize}X |}
 \hline
  \scriptsize Measurement & \scriptsize Simulation & \scriptsize Ray tracing & \scriptsize Open Dataset \\
 \hline
 ~\cite{alteredAP,8651736,7743685,MonoDCell,vlfANN,7938617,OnDevice,lorawan,telco,6805641,wsn_svr,RadioMaps,tlfcma,LowOverhead,magnetic_inertial,IndustrialWSN,uav,location_aware,8240410,8108573,OpticalCamera,devicefree,10.1145/3321408.3321584,8780770,8673800,rfid,kmgpr,8765368,Discriminative,DataAugmentation,8362712,Eloc,HumanDetection,RelationLearning,FullBandGSM,grof,hapi,hiwl,7064997,WeightedAmbientWiFi,eee112,8008794,8584443,JUIndoorLoc,7313038,8931646,LiUnsupervised,yang2012locating,8115921,8661625,Wang2017WiFiFB,Chunjing2017WLAN,8422182,wu2019mobile,feng2019received,zhang2017efficient,xu2019efficient,cottone2016machine, sun2008adaptive,khatab2017fingerprint,yan2018noise,wang2019robust,mei2018novel,wu2018accurate,nguyen2017performance,musa2019decision,zou2015fast,rezgui2017efficient,figuera2012advanced,guo2018accurate,bi2018adaptive,elbes2019indoor,comiter2018localization,liu2019hybrid,liu2017wicount,ahmadi2017exploiting,adege2018indoor,adege2019mobility,schmidt2019sdr,gu2015online,yang2018clustering,yan2017hybrid,malik2019indoor,bae2019large,tewes2019ensemble,sung2019neural,li2017measurement,sanam2018improved,xiao2012large,zhao2019accurate,salamah2016enhanced,widmaier2019towards,homayounvala2019novel,zhang2019improving,belmonte2019swiblux,dashti2016extracting,yang2012locating,oussar2011indoor,chen2019dpr,mahfouz2015kernel,qiu2018walk,van2015machine_1,niitsoo2019deep_2,wang2016csi_3,wang2016csi_5,wu2019csi_7,li2018channel_8,wang2017cifi_9,niitsoo2018convolutional_11,li2019convolutional_12,rizk2018cellindeep_15,aikawa2019cnn_16,wang2018deep_23,hsieh2019deep_28,li2019deep_31,gan2017deep_32,wang2015deepfi_33,yazdanian2018deeppos_34,berruet2018delfin_35,xue2019deeptal_36,zhang2016deep_38,wang2017biloc_42,wu2017passive_44,ghourchian2017real_45} ~\cite{zhou2017robust_46,sorour2014joint_47,zhang2020transfer_49,shokry2018deeploc_50,ouyang2011indoor_51,liu2009low_52,gu2015semi_54,pulkkinen2011semi,zhou2017semi_55,wang2017resloc_56,aikawa2018wlan_61,abbas2019wideep_63,huang2020widet_64 , chen2019wifi, dayekh2010cooperative_66 ,kram2019uwb_68,choi2019unsupervised_69,krishnan2018improving_71,alhajri2019indoor_74,goswami2011wigem_75,zhou2017grassma_76,decurninge2018csi_81,arnold2018deep_82,zhou2017indoor_86,chen2018deep_88,jung2015unsupervised_89,sen2012you_91,wang2012no_92,wu2012will_93,ray2016localization_94,lee2018dnn_95,rizk2019device_96,rizk2019solocell_98,wang2018deepmap_103,liu2018autloc_104,zhang2017deeppositioning_106,tarekegn2019applying_107,zhang2019deeploc_108,mittal2018adapting_109,adege2018applying_113,sobehy2019csi_117,song2019novel_119,shao2018indoor_120,de2019csi_121,choi2019unsupervised_123,own2019signal_125,ebuchi2019vehicle_126,pandey2019handling_127,de2019enhanced_129} 
 
 
 
 & ~\cite{FPfusing,InterpretingCNN,MLthesis,MassiveMIMO,7504333,NLOS_UWB,sdr,TargetTracking,tdoa,patent,FineGrainedSubcarrier,ZhangIndoor,8712551,AntonioLocalization,jaafar2018neural,ge2019hybrid} \cite{felix2016fingerprinting,comiter2017data,comiter2017structured,zou2015fast,comiter2018localization,zhang2018heterogeneous,yi2019neural,bhatti2018machine,xiao2018learning,mahfouz2015kernel,njima2019deep_22,chen2011semi_53,li2017robust_60,prasad2018machine_62,vieira2017deep_80,prasad2017numerical_84,pirzadeh2019machine_87,sun2018single_90,chen2018multipath_111,xiong2019decorrelation_115,wu2019neural_116,own2019signal_125,lei2019siamese_130} 
 
 & ~\cite{mmwave,AntonioLocalization,gan2017deep_32,butt2020rf_57,wang2019fast_83,de2019enhanced_129,bekkali2011gaussian} 
 
 & ~\cite{mmwave,gbrbm,kmgpr,Timotheatos2017FeatureEA,FeatureSelection,hybloc,Qian2019Supervised,wang2019robust,nguyen2017performance,zhang2018enhancement,tewes2019ensemble,kim2018hybrid,xiao2018learning,patel2020millimeter,qian2019convolutional_10,ibrahim2018cnn_13,turgut2019deep_27,wang2020robust_59,ciftler2020federated_70,jang2018indoor_99,nowicki2017low,belmannoubi2019stacked_110,dou2018top_112,song2019novel_119} ~\cite{csiRNN,kim2018scalable,secckin2019hierarchical,li2019smartloc}\\
 %\hline
 %Code available online &  &  &  & ~\cite{csiRNN,kim2018scalable,secckin2019hierarchical}\\
 \hline
\end{tabularx}
\end{scriptsize}
\end{tiny}
\caption{Test data}
\label{tab:Dataset}
\end{table}
% removed cheng2018fingerprint

==> AllTables/DatasetTable.tex <==
\begin{center}
    \begin{longtable}{|p{3cm}|p{2cm}|p{3cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
        \hline
        Dataset name & Date released & Features used & Wireless Technology used & Location points & Available online? & Environment\\
        \hline
        \hline
        \endfirsthead
        \hline
        Dataset name & Date released & Features used & Wireless Technology used & Location points & Available online? & Environment\\
        \hline
        \hline
        \endhead
        Long-Term Wifi Fingerprinting Dataset ~\cite{ref1} & November 24, 2017 & RSSI, location coordinates & Wi-fi & 212 reference points with 63,504 measurements & Yes ~\cite{mendoza_silva_german_martin_2017_1066041} & Indoor (Multi-floor) \\
        \hline
        Wifi Crowdsourced Fingerprinting Dataset ~\cite{ref2} & September 12, 2017 & RSSI, local location coordinates & Wi-fi & 4648 fingerprints & Yes ~\cite{lohan_elena_simona_2017_889798} & Indoor (Multi-floor) \\
        \hline
        WLAN Indoor Ranging Dataset ~\cite{ref3} & 2018 & WLAN Ranging Signals & WLAN & Approx. 320 files each with a 300x30000 MATLAB Matrix & Yes ~\cite{wlan_indoor_ranging_dataset} & Indoor \\
        \hline
        RFKON Anchor-based Data-set ~\cite{ref4} & 2016 & Wi-fi RSS, Bluetooth RSS, BLE RSS, Link Quality Indicators & Wi-fi, Bluetooth & 54 reference points & Not available (link in paper says access forbidden) & Multi-floor \\
        \hline
        RFKON Mobile-based Data-set ~\cite{ref4} & 2016 & Wi-fi RSS, Bluetooth RSS, Magnetometer readings, Accelerometer readings & Wi-fi, Bluetooth & 54 reference points & Not available (link in paper says access forbidden) & Multi-floor \\
        \hline
        Rural Sigfox data-set ~\cite{ref5} & March 7, 2018 & RSSI, Location coordinates & Low Power WAN & 25,638 rows & Yes ~\cite{aernouts_michiel_2018_1193563} & Outdoor \\
        \hline
        Urban Sigfox data-set ~\cite{ref5} & March 7, 2018 & RSSI, Location coordinates & Low Power WAN & 14,378 rows & Yes ~\cite{aernouts_michiel_2018_1193563} & Outdoor \\
        \hline
        Urban LoRaWAN data-set ~\cite{ref5} & March 7, 2018 & RSSI, Location coordinates, Low Range Spreading Factor (SF), Horizontal Dilution of Precision (HDOP) & Low Power WAN & 123,529 rows & Yes ~\cite{aernouts_michiel_2018_1193563} & Outdoor \\
        \hline
        Residential wearable RSSI and accelerometer measurements dataset ~\cite{ref6} & June 12, 2018 &  RSSI, accelerometer readings, battery level of wearable devices, tagged video of user & Wi-fi & 42 MB of csv files & Yes ~\cite{Byrne2018} & Indoor (4 different residences) \\
        \hline
        UJIIndoorLoc-Mag ~\cite{ref7} & September 10, 2015 & Magentometer readings, Accelerometer readings and Rotation Sensor readings, Location coordinates & None (Sensor readings only) & 40,159 measurements & Yes ~\cite{Dua:2019, UJIIndoorLoc_Mag} & Indoor \\
        \hline
        UJIIndoorLoc ~\cite{ref8} & September 18, 2014 & RSSI from 520 APs, Location co-ordinates & Wi-fi & 933 different locations, 21049 different readings & Yes~\cite{Dua:2019, UJIIndoorLoc} & Multi-building, Multi-floor\\
        \hline
        AmbiLoc ~\cite{ref9} & September 18, 2017 & RSSI from FM, TV and GSM signals, coordinates & FM Radio, TV, GSM & 2697 samples & Yes ~\cite{AmbiLoc} & Multi-building, Multi-floor \\
        \hline
        PerfLoc ~\cite{ref10} & September 2016 & Motion sensors, RSSI from Wifi and Cellular, GPS & Wi-fi, Cellular & 900 points & Yes & Multi-building, Multi-floor \\
        \hline
        KIOS Dataset ~\cite{ref11} & 2013 & RSSI from all available APs & Wi-fi & 105 different reference points, 2100 fingerprints & Yes ~\cite{KIOS} & Indoor \\
        \hline
        BLE RSS Measurements Dataset ~\cite{ref12} & December 5, 2018 & RSS from BLE Beacons, coordinates & BLE & 4752 different samples & Yes ~\cite{mendoza_silva_german_martin_2018_1618692} & Indoor (2 university zones) \\
        \hline
        MagPIE ~\cite{ref13} & September 2017 & Accelerometer, Gyroscope, Magnetometer readings& None(Only IMU and Magnetometer) & 13 hours of data & Yes ~\cite{MagPIE} & Multi-building\\
        \hline
        JUIndoorLoc ~\cite{ref14} & February 2019 & RSSI Data & Wi-fi & 25,364 samples & Yes ~\cite{JUIndoorLoc} & Multi-floor \\
        \hline
        XJTLUIndoorLoc ~\cite{ref15} & November 2018 & RSSI from Wi-fi, Geomagnetic field strength and Rotation Sensor readings& Wi-fi& 969 reference points & No & Multi-floor\\
        \hline
    \end{longtable}
\end{center}

==> AllTables/DatasetTable2.tex <==

\begin{strip}
\begin{footnotesize}
\begin{tabularx}{1\textwidth}
 { 
  | >{\raggedleft\arraybackslash\hsize=1.5\hsize}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash}X |}

 \hline
 \caption{Dataset Table}
 {\bf Dataset name & \bf Date released & \bf Features used & \bf Wireless Technology & \bf Location points & \bf Availability online  & \bf  Environment} \\
 \hline
 Long-Term WiFi Fingerprinting Dataset ~\cite{ref1} & November, 2017 & RSSI, location coordinates & WiFi & 212 reference points with 63,504 measurements & Yes ~\cite{mendoza_silva_german_martin_2017_1066041} & Indoor (Multi-floor) \\
 \hline
 WiFi Crowdsourced Fingerprinting Dataset ~\cite{ref2} & September, 2017 & RSSI, local location coordinates & WiFi & 4648 fingerprints & Yes ~\cite{lohan_elena_simona_2017_889798} & Indoor (Multi-floor) \\
 \hline
 WLAN Indoor Ranging Dataset ~\cite{ref3} & 2018 & WLAN Ranging Signals & WLAN & Approx. 320 files each with a 300x30000 MATLAB Matrix & Yes ~\cite{wlan_indoor_ranging_dataset} & Indoor \\
 \hline
 RFKON Anchor-based Data-set ~\cite{ref4} & 2016 & WiFi RSS, Bluetooth RSS, BLE RSS, Link Quality Indicators & WiFi, Bluetooth & 54 reference points &   Access forbidden) & Multi-floor \\
 \hline
 RFKON Mobile-based Data-set ~\cite{ref4} & 2016 & WiFi RSS, Bluetooth RSS, Magnetometer readings, Accelerometer readings & WiFi, Bluetooth & 54 reference points & Access forbidden) & Multi-floor \\
 \hline
 Rural Sigfox data-set ~\cite{ref5} & March, 2018 & RSSI, Location coordinates & Low Power WAN & 25,638 rows & Yes ~\cite{aernouts_michiel_2018_1193563} & Outdoor \\
 \hline
 Urban Sigfox data-set ~\cite{ref5} & March, 2018 & RSSI, Location coordinates & Low Power WAN & 14,378 rows & Yes ~\cite{aernouts_michiel_2018_1193563} & Outdoor \\
 \hline
 Urban LoRaWAN data-set ~\cite{ref5} & March, 2018 & RSSI, Location coordinates, Low Range Spreading Factor (SF), Horizontal Dilution of Precision (HDOP) & Low Power WAN & 123,529 rows & Yes ~\cite{aernouts_michiel_2018_1193563} & Outdoor \\
 \hline
 Residential wearable RSSI and accelerometer measurements dataset ~\cite{ref6} & June, 2018 &  RSSI, accelerometer readings, battery level of wearable devices, tagged video of user & WiFi & 42 MB of csv files & Yes ~\cite{Byrne2018} & Indoor (4 different residences) \\
        \hline
        UJIIndoorLoc-Mag ~\cite{ref7} & September, 2015 & Magentometer readings, Accelerometer readings and Rotation Sensor readings, Location coordinates & None (Sensor readings only) & 40,159 measurements & Yes ~\cite{Dua:2019, UJIIndoorLoc_Mag} & Indoor \\
        \hline
        UJIIndoorLoc ~\cite{ref8} & September, 2014 & RSSI from 520 APs, Location co-ordinates & WiFi & 933 different locations, 21049 different readings & Yes~\cite{Dua:2019, UJIIndoorLoc} & Multi-building, Multi-floor\\
        \hline
        AmbiLoc ~\cite{ref9} & September, 2017 & RSSI from FM, TV and GSM signals, coordinates & FM Radio, TV, GSM & 2697 samples & Yes ~\cite{AmbiLoc} & Multi-building, Multi-floor \\
        \hline
        PerfLoc ~\cite{ref10} & September, 2016 & Motion sensors, RSSI from WiFi and Cellular, GPS & WiFi, Cellular & 900 points & Yes & Multi-building, Multi-floor \\
        \hline
        KIOS Dataset ~\cite{ref11} & 2013 & RSSI from all available APs & WiFi & 105 different reference points, 2100 fingerprints & Yes ~\cite{KIOS} & Indoor \\
        \hline
        BLE RSS Measurements Dataset ~\cite{ref12} & December, 2018 & RSS from BLE Beacons, coordinates & BLE & 4752 different samples & Yes ~\cite{mendoza_silva_german_martin_2018_1618692} & Indoor (2 university zones) \\
        %\hline
        %MagPIE ~\cite{ref13} & September 2017 & Accelerometer, Gyroscope, Magnetometer readings& None(Only IMU and Magnetometer) & 13 hours of data & Yes ~\cite{MagPIE} & Multi-building\\
        \hline
        JUIndoorLoc ~\cite{ref14} & February 2019 & RSSI Data & WiFi & 25,364 samples & Yes ~\cite{JUIndoorLoc} & Multi-floor \\
        \hline
        XJTLUIndoor-Loc ~\cite{ref15} & November 2018 & RSSI from WiFi, Geomagnetic field strength and Rotation Sensor readings& WiFi& 969 reference points & No & Multi-floor\\
 \hline
\end{tabularx}
\end{footnotesize}
\end{strip}

==> AllTables/DatasetTable3.tex <==
\begin{table*}
\begin{scriptsize}
    \centering
    \begin{tabular}{|p{3cm}|p{2cm}|p{3cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
      %  \hline
%        Dataset name & Date released & Features used & Wireless Technology used & Location points & Available online? & Environment\\
      %  \hline
        \hline
        Dataset name & Date released & Features used & Wireless Technology used & Location points & Online Availability & Environment\\
        \hline
        Long-Term WiFi Fingerprinting Dataset ~\cite{ref1} & November, 2017 & RSSI, location coordinates & WiFi & 212 reference points with 63,504 measurements & Yes ~\cite{mendoza_silva_german_martin_2020_3748719} & Indoor (Multi-floor) \\
        \hline
        WiFi Crowdsourced Fingerprinting Dataset ~\cite{ref2} & September, 2017 & RSSI, local location coordinates & WiFi & 4648 fingerprints & Yes ~\cite{lohan_elena_simona_2017_889798} & Indoor (Multi-floor) \\
        \hline
        WLAN Indoor Ranging Dataset ~\cite{ref3} & 2018 & WLAN Ranging Signals & WLAN (IEEE 802.11g/n) & Approx. 320 files each with a 300x30000 MATLAB Matrix & Yes ~\cite{wlan_indoor_ranging_dataset} & Indoor \\
        \hline
        RFKON Anchor-based Data-set ~\cite{ref4} & 2016 & WiFi RSS, Bluetooth RSS, BLE RSS, Link Quality Indicators & WiFi, Bluetooth & 54 reference points & Link failure & Multi-floor \\
        \hline
        RFKON Mobile-based Data-set ~\cite{ref4} & 2016 & WiFi RSS, Bluetooth RSS, Magnetometer readings, Accelerometer readings & WiFi, Bluetooth & 54 reference points & Link failure & Multi-floor \\
        \hline
        Rural Sigfox data-set ~\cite{ref5} & March, 2018 & RSSI, Location coordinates & Low Power WAN (Sigfox) & 25,638 rows & Yes ~\cite{aernouts_michiel_2018_1193563} & Outdoor \\
        \hline
        Urban Sigfox data-set ~\cite{ref5} & March, 2018 & RSSI, Location coordinates & Low Power WAN (LoRaWAN) & 14,378 rows & Yes ~\cite{aernouts_michiel_2018_1193563} & Outdoor \\
        \hline
        Urban LoRaWAN data-set ~\cite{ref5} & March, 2018 & RSSI, Location coordinates, Low Range Spreading Factor (SF), Horizontal Dilution of Precision (HDOP) & Low Power WAN (LoRaWAN) & 123,529 rows & Yes ~\cite{aernouts_michiel_2018_1193563} & Outdoor \\
        \hline
        Residential wearable RSSI and accelerometer measurements dataset ~\cite{ref6} & June, 2018 &  RSSI, accelerometer readings, battery level of wearable devices, tagged video of user & BLE (Bluetooth 4.0) & 42 MB of csv files & Yes ~\cite{Byrne2018} & Indoor (4 different residences) \\
        \hline
        UJIIndoorLoc-Mag ~\cite{ref7} & September, 2015 & Magentometer readings, Accelerometer readings and Rotation Sensor readings, Location coordinates & None (Sensor readings only) & 40,159 measurements & Yes ~\cite{Dua:2019, UJIIndoorLoc_Mag} & Indoor \\
        \hline
        UJIIndoorLoc ~\cite{ref8} & September, 2014 & RSSI from 520 APs, Location co-ordinates & WiFi & 933 different locations, 21049 different readings & Yes~\cite{Dua:2019, UJIIndoorLoc} & Multi-building, Multi-floor\\
        \hline
        AmbiLoc ~\cite{ref9} & September, 2017 & RSSI from FM, TV and GSM signals, coordinates & FM Radio, TV, GSM & 2697 samples & Yes ~\cite{AmbiLoc} & Multi-building, Multi-floor \\
        \hline
        PerfLoc ~\cite{ref10} & September, 2016 & Motion sensors, RSSI from WiFi and Cellular, GPS & WiFi, Cellular & 900 points & Yes & Multi-building, Multi-floor \\
        \hline
        KIOS Dataset ~\cite{ref11} & 2013 & RSSI from all available APs & WiFi & 105 different reference points, 2100 fingerprints & Yes ~\cite{KIOS} & Indoor \\
        \hline
        BLE RSS Measurements Dataset ~\cite{ref12} & December, 2018 & RSS from BLE Beacons, coordinates & BLE (Bluetooth 4.0) & 4752 different samples & Yes ~\cite{mendoza_silva_german_martin_2018_1618692} & Indoor (2 university zones) \\
        \hline
        MagPIE ~\cite{ref13} & September, 2017 & Accelerometer, Gyroscope, Magnetometer readings& None(Only IMU and Magnetometer) & 13 hours of data & Yes ~\cite{MagPIE} & Multi-building\\
        \hline
        JUIndoorLoc ~\cite{ref14} & February, 2019 & RSSI Data & WiFi & 25,364 samples & Yes ~\cite{JUIndoorLoc} & Multi-floor \\
        \hline
        XJTLUIndoorLoc ~\cite{ref15} & November, 2018 & RSSI from WiFi, Geomagnetic field strength and Rotation Sensor readings& WiFi& 969 reference points & No & Multi-floor\\
        \hline
    \end{tabular}
    \end{scriptsize}
    \end{table*}

==> AllTables/LearningTypeTbl.tex <==
\begin{tabularx}{\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=.75\hsize}X |}
 \caption{Type of ML model used}
 \hline
  & Supervised & Semi-Supervised & Unsuperv-ised & Other \\
 \hline
 Standard ML & ~\cite{alteredAP} ~\cite{FPfusing} ~\cite{InterpretingCNN} ~\cite{7504333} ~\cite{msvr} ~\cite{7938617} ~\cite{NLOS_UWB} ~\cite{6488858} ~\cite{OnDevice} ~\cite{telco} ~\cite{sdr} ~\cite{6805641} ~\cite{TargetTracking} ~\cite{tdoa} ~\cite{RadioMaps} ~\cite{magnetic_inertial} ~\cite{IndustrialWSN} ~\cite{uav} ~\cite{patent} ~\cite{mmwave} ~\cite{8240410} ~\cite{8108573} ~\cite{OpticalCamera} ~\cite{manifold} ~\cite{probabilistic_localization} ~\cite{gbrbm} ~\cite{8780770} ~\cite{8673800} ~\cite{rfid} ~\cite{kmgpr} ~\cite{DNN/KNN} ~\cite{Discriminative} ~\cite{8362712} ~\cite{FineGrainedSubcarrier} ~\cite{Timotheatos2017FeatureEA} ~\cite{FeatureSelection} ~\cite{FullBandGSM} ~\cite{grof} ~\cite{hapi} ~\cite{hybloc} ~\cite{7064997} ~\cite{WeightedAmbientWiFi} ~\cite{eee112} ~\cite{8008794} ~\cite{8584443} ~\cite{8543713} ~\cite{DricotModular} ~\cite{JUIndoorLoc} ~\cite{7313038} ~\cite{8931646} ~\cite{7996460} ~\cite{yang2012locating} ~\cite{zhang2017efficient} ~\cite{cottone2016machine} \cite{cheng2018fingerprint} ~\cite{mei2018novel} ~\cite{wu2018accurate} ~\cite{hossan2018novel} ~\cite{nguyen2017performance} ~\cite{musa2019decision} ~\cite{rezgui2017efficient} ~\cite{afzal2014localization} ~\cite{figuera2012advanced} ~\cite{guo2018accurate} ~\cite{bi2018adaptive} ~\cite{lee2013new} ~\cite{wang2007agent} ~\cite{zhang2018heterogeneous} ~\cite{ahmadi2017exploiting} ~\cite{adege2018indoor} ~\cite{yan2017hybrid} ~\cite{li2017measurement} ~\cite{sanam2018improved} ~\cite{salamah2016enhanced} ~\cite{homayounvala2019novel} ~\cite{bhatti2018machine} ~\cite{savic2014kernel} ~\cite{zhang2019improving} ~\cite{tran2008localization} ~\cite{secckin2019hierarchical} ~\cite{feng2010location} ~\cite{li2019smartloc} ~\cite{dashti2016extracting} ~\cite{livinsa2015localization} ~\cite{yang2012locating} ~\cite{oussar2011indoor} ~\cite{mahfouz2015kernel} ~\cite{yan2015improved} & ~\cite{laperls} ~\cite{8651736} ~\cite{MassiveMIMO} ~\cite{7743685} ~\cite{wsn_svr} ~\cite{IndoorOutdoor} ~\cite{ZhangIndoor} ~\cite{8115921} ~\cite{LiUnsupervised}  ~\cite{Chunjing2017WLAN} ~\cite{chen2019dpr} & ~\cite{location_aware} ~\cite{dabil} ~\cite{gbrbm} ~\cite{hiwl} ~\cite{li2019smartloc} & ~\cite{tlfcma} ~\cite{LowOverhead} ~\cite{8661625} ~\cite{feng2019received} \cite{sun2008adaptive} ~\cite{guo2018accurate} ~\cite{yang2018clustering} ~\cite{xiao2012large} ~\cite{qiu2018walk}\\
 \hline
 Deep conv based & ~\cite{Eloc} ~\cite{DCNN} ~\cite{Qian2019Supervised} ~\cite{Zhang2019Wireless} ~\cite{comiter2018localization} ~\cite{liu2019hybrid} ~\cite{schmidt2019sdr} ~\cite{al2018improved} ~\cite{zhang2018enhancement} ~\cite{tewes2019ensemble} ~\cite{zhou2019smartphone} ~\cite{zhao2019accurate} ~\cite{patel2020millimeter} &  &  & \\
 \hline
 Deep recurrent & ~\cite{MLthesis} ~\cite{MonoDCell} ~\cite{vlfANN} ~\cite{telco} ~\cite{Qian2019Supervised} ~\cite{uav} ~\cite{csiRNN} ~\cite{wu2019mobile} ~\cite{xu2019efficient} ~\cite{yan2018noise} ~\cite{elbes2019indoor} ~\cite{adege2019mobility} ~\cite{bae2019large} ~\cite{wang2019indoor} ~\cite{patel2020millimeter} &  &  & \\
 \hline
 Deep Other & ~\cite{sdr} ~\cite{DNN/KNN} ~\cite{HumanDetection} ~\cite{Timotheatos2017FeatureEA} ~\cite{RelationLearning} ~\cite{hapi} ~\cite{mmbp} ~\cite{8584443} ~\cite{8543713} ~\cite{RamaLocalization} ~\cite{Wang2017WiFiFB} ~\cite{8422182} ~\cite{jaafar2018neural} ~\cite{pelka2018new} ~\cite{ge2019hybrid} \cite{felix2016fingerprinting} ~\cite{khatab2017fingerprint} ~\cite{kim2018scalable} ~\cite{wang2019robust} ~\cite{mei2018novel} ~\cite{comiter2017data} ~\cite{comiter2017structured} ~\cite{banihashemian2019new} ~\cite{guo2018accurate} ~\cite{liu2017wicount} ~\cite{adege2018indoor} ~\cite{schmidt2019sdr} ~\cite{malik2019indoor} ~\cite{yi2019neural} ~\cite{sung2019neural} ~\cite{kim2018hybrid} ~\cite{widmaier2019towards} ~\cite{belmonte2019swiblux} ~\cite{xiao2018learning} & ~\cite{8651736} ~\cite{lorawan} ~\cite{10.1145/3321408.3321584} ~\cite{DataAugmentation} ~\cite{Qian2019Supervised} & ~\cite{pseudolite} & ~\cite{lorawan} ~\cite{khatab2017fingerprint} ~\cite{zou2015fast} ~\cite{gu2015online}\\
 \hline
\end{tabularx}
\newpage

==> AllTables/LearningTypeTbl2.tex <==
\begin{tabularx}{\textwidth}{lX} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=.75\hsize}X |}
 \caption{Type of ML model used}
 \label{tab:MLType}
 \hline
  & Supervised & Semi-Supervised & Unsupervised & Other \\
 \hline
 Standard ML & ~\cite{alteredAP} ~\cite{FPfusing} ~\cite{InterpretingCNN} ~\cite{7504333} ~\cite{7938617} ~\cite{NLOS_UWB} ~\cite{OnDevice} ~\cite{telco} ~\cite{sdr} ~\cite{6805641} ~\cite{TargetTracking} ~\cite{tdoa} ~\cite{RadioMaps} ~\cite{magnetic_inertial} ~\cite{IndustrialWSN} ~\cite{uav} ~\cite{patent} ~\cite{mmwave} ~\cite{8240410} ~\cite{8108573} ~\cite{OpticalCamera} ~\cite{probabilistic_localization} ~\cite{gbrbm} ~\cite{8780770} ~\cite{8673800} ~\cite{rfid} ~\cite{kmgpr} ~\cite{DNN/KNN} ~\cite{Discriminative} ~\cite{8362712} ~\cite{FineGrainedSubcarrier} ~\cite{Timotheatos2017FeatureEA} ~\cite{FeatureSelection} ~\cite{FullBandGSM} ~\cite{grof} ~\cite{hapi} ~\cite{hybloc} ~\cite{7064997} ~\cite{WeightedAmbientWiFi} ~\cite{eee112} ~\cite{8008794} ~\cite{8584443} ~\cite{JUIndoorLoc} ~\cite{7313038} ~\cite{8931646} ~\cite{yang2012locating} ~\cite{zhang2017efficient} ~\cite{cottone2016machine} \cite{cheng2018fingerprint} ~\cite{mei2018novel} ~\cite{wu2018accurate} ~\cite{nguyen2017performance} ~\cite{musa2019decision} ~\cite{rezgui2017efficient} ~\cite{figuera2012advanced} ~\cite{guo2018accurate} ~\cite{bi2018adaptive} ~\cite{zhang2018heterogeneous} ~\cite{ahmadi2017exploiting} ~\cite{adege2018indoor} ~\cite{yan2017hybrid} ~\cite{li2017measurement} ~\cite{sanam2018improved} ~\cite{salamah2016enhanced} ~\cite{homayounvala2019novel} ~\cite{bhatti2018machine} ~\cite{zhang2019improving} ~\cite{secckin2019hierarchical} ~\cite{li2019smartloc} ~\cite{dashti2016extracting} ~\cite{yang2012locating} ~\cite{oussar2011indoor} ~\cite{mahfouz2015kernel} & ~\cite{laperls} ~\cite{8651736} ~\cite{MassiveMIMO} ~\cite{7743685} ~\cite{wsn_svr} ~\cite{ZhangIndoor} ~\cite{8115921} ~\cite{LiUnsupervised}  ~\cite{Chunjing2017WLAN} ~\cite{chen2019dpr} & ~\cite{location_aware} ~\cite{dabil} ~\cite{gbrbm} ~\cite{hiwl} ~\cite{li2019smartloc} & ~\cite{tlfcma} ~\cite{LowOverhead} ~\cite{8661625} ~\cite{feng2019received} \cite{sun2008adaptive} ~\cite{guo2018accurate} ~\cite{yang2018clustering} ~\cite{xiao2012large} ~\cite{qiu2018walk}\\
 \hline
 Deep conv based & ~\cite{Eloc} ~\cite{DCNN} ~\cite{Qian2019Supervised} ~\cite{Zhang2019Wireless} ~\cite{comiter2018localization} ~\cite{liu2019hybrid} ~\cite{schmidt2019sdr} ~\cite{zhang2018enhancement} ~\cite{tewes2019ensemble} ~\cite{zhao2019accurate} ~\cite{patel2020millimeter} &  &  & \\
 \hline
 Deep recurrent & ~\cite{MLthesis} ~\cite{MonoDCell} ~\cite{vlfANN} ~\cite{telco} ~\cite{Qian2019Supervised} ~\cite{uav} ~\cite{csiRNN} ~\cite{wu2019mobile} ~\cite{xu2019efficient} ~\cite{yan2018noise} ~\cite{elbes2019indoor} ~\cite{adege2019mobility} ~\cite{bae2019large} ~\cite{patel2020millimeter} &  &  & \\
 \hline
 Deep Other & ~\cite{sdr} ~\cite{DNN/KNN} ~\cite{HumanDetection} ~\cite{Timotheatos2017FeatureEA} ~\cite{RelationLearning} ~\cite{hapi} ~\cite{mmbp} ~\cite{8584443} ~\cite{RamaLocalization} ~\cite{Wang2017WiFiFB} ~\cite{8422182} ~\cite{jaafar2018neural} ~\cite{ge2019hybrid} \cite{felix2016fingerprinting} ~\cite{khatab2017fingerprint} ~\cite{kim2018scalable} ~\cite{wang2019robust} ~\cite{mei2018novel} ~\cite{comiter2017data} ~\cite{comiter2017structured} ~\cite{guo2018accurate} ~\cite{liu2017wicount} ~\cite{adege2018indoor} ~\cite{schmidt2019sdr} ~\cite{malik2019indoor} ~\cite{yi2019neural} ~\cite{sung2019neural} ~\cite{kim2018hybrid} ~\cite{widmaier2019towards} ~\cite{belmonte2019swiblux} ~\cite{xiao2018learning} & ~\cite{8651736} ~\cite{lorawan} ~\cite{10.1145/3321408.3321584} ~\cite{DataAugmentation} ~\cite{Qian2019Supervised} & & ~\cite{lorawan} ~\cite{khatab2017fingerprint} ~\cite{zou2015fast} ~\cite{gu2015online}\\
 \hline
\end{tabularx}

==> AllTables/LearningTypeTbl3.tex <==
\begin{tabularx}{0.5\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=.75\hsize}X |}
 \caption{Type of ML model used}
  \label{tab:MLType}
 \hline
  & Supervised & Semi-Supervised & Unsupervised & Other \\
 \hline
 Standard ML & ~\cite{alteredAP,FPfusing,InterpretingCNN,7504333,7938617,NLOS_UWB,OnDevice,telco,sdr,6805641,TargetTracking,tdoa,RadioMaps,magnetic_inertial,IndustrialWSN,uav,patent,mmwave,8240410,8108573,OpticalCamera,probabilistic_localization,gbrbm,8780770,8673800,rfid,kmgpr,DNN/KNN,Discriminative,8362712,FineGrainedSubcarrier,Timotheatos2017FeatureEA,FeatureSelection,FullBandGSM,grof,hapi,hybloc,7064997,WeightedAmbientWiFi,eee112,8008794,8584443,JUIndoorLoc,7313038,8931646,yang2012locating,zhang2017efficient,cottone2016machine} \cite{cheng2018fingerprint,mei2018novel,wu2018accurate,nguyen2017performance,musa2019decision,rezgui2017efficient,figuera2012advanced,guo2018accurate,bi2018adaptive,zhang2018heterogeneous,ahmadi2017exploiting,adege2018indoor,yan2017hybrid,li2017measurement,sanam2018improved,salamah2016enhanced,homayounvala2019novel,bhatti2018machine,zhang2019improving,secckin2019hierarchical,li2019smartloc,dashti2016extracting,yang2012locating,oussar2011indoor,mahfouz2015kernel} & ~\cite{laperls,8651736,MassiveMIMO,7743685,wsn_svr,ZhangIndoor,8115921,LiUnsupervised}  ~\cite{Chunjing2017WLAN,chen2019dpr} & ~\cite{location_aware,dabil,gbrbm,hiwl,li2019smartloc} & ~\cite{tlfcma,LowOverhead,8661625,feng2019received} \cite{sun2008adaptive,guo2018accurate,yang2018clustering,xiao2012large,qiu2018walk}\\
 \hline
 Deep conv based & ~\cite{Eloc,DCNN,Qian2019Supervised,Zhang2019Wireless,comiter2018localization,liu2019hybrid,schmidt2019sdr,zhang2018enhancement,tewes2019ensemble,zhao2019accurate,patel2020millimeter} &  &  & \\
 \hline
 Deep recurrent & ~\cite{MLthesis,MonoDCell,vlfANN,telco,Qian2019Supervised,uav,csiRNN,wu2019mobile,xu2019efficient,yan2018noise,elbes2019indoor,adege2019mobility,bae2019large,patel2020millimeter} &  &  & \\
 \hline
 Deep Other & ~\cite{sdr,DNN/KNN,HumanDetection,Timotheatos2017FeatureEA,RelationLearning,hapi,mmbp,8584443,RamaLocalization,Wang2017WiFiFB,8422182,jaafar2018neural,ge2019hybrid} \cite{felix2016fingerprinting,khatab2017fingerprint,kim2018scalable,wang2019robust,mei2018novel,comiter2017data,comiter2017structured,guo2018accurate,liu2017wicount,adege2018indoor,schmidt2019sdr,malik2019indoor,yi2019neural,sung2019neural,kim2018hybrid,widmaier2019towards,belmonte2019swiblux,xiao2018learning} & ~\cite{8651736,lorawan,10.1145/3321408.3321584,DataAugmentation,Qian2019Supervised} & & ~\cite{lorawan,khatab2017fingerprint,zou2015fast,gu2015online}\\
 \hline
\end{tabularx}

==> AllTables/LearningTypeTbl4.tex <==
\begin{table}
\begin{tiny}
\begin{tabularx}{0.45\textwidth} { 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \hline
  & \tiny Supervised & \tiny Semi-Supervised & \tiny Unsupervised  & \tiny Other \\
 \hline
 Standard ML & ~\cite{alteredAP,FPfusing,InterpretingCNN,7504333,7938617,NLOS_UWB,OnDevice,telco,sdr,6805641,TargetTracking,tdoa,RadioMaps,magnetic_inertial,IndustrialWSN,uav,patent,mmwave,8240410,8108573,OpticalCamera,probabilistic_localization,gbrbm,8780770,8673800,rfid,kmgpr,DNN/KNN,Discriminative,8362712,FineGrainedSubcarrier,Timotheatos2017FeatureEA,FeatureSelection,FullBandGSM,grof,hapi,hybloc,7064997,WeightedAmbientWiFi,eee112,8008794,8584443,JUIndoorLoc,7313038,8931646,yang2012locating,zhang2017efficient,cottone2016machine} \cite{mei2018novel,wu2018accurate,nguyen2017performance,musa2019decision,rezgui2017efficient,figuera2012advanced,guo2018accurate,bi2018adaptive,zhang2018heterogeneous,ahmadi2017exploiting,adege2018indoor,yan2017hybrid,li2017measurement,sanam2018improved,salamah2016enhanced,homayounvala2019novel,bhatti2018machine,zhang2019improving,secckin2019hierarchical,li2019smartloc,dashti2016extracting,yang2012locating,oussar2011indoor,mahfouz2015kernel,roshanaei2009dynamic,ma2008cluster,roshanaei2009dynamic,torteeka2014indoor,peng2016iterative} & ~\cite{laperls,8651736,MassiveMIMO,7743685,wsn_svr,ZhangIndoor,8115921,LiUnsupervised}  ~\cite{Chunjing2017WLAN,chen2019dpr} & ~\cite{location_aware,dabil,gbrbm,hiwl,li2019smartloc} & ~\cite{tlfcma,LowOverhead,8661625,feng2019received} \cite{sun2008adaptive,guo2018accurate,yang2018clustering,xiao2012large,qiu2018walk}\\
 \hline
Convolutional based & ~\cite{Eloc,DCNN,Qian2019Supervised,Zhang2019Wireless,comiter2018localization,liu2019hybrid,schmidt2019sdr,zhang2018enhancement,tewes2019ensemble,zhao2019accurate,patel2020millimeter} &  &  & \\
 \hline
Recurrent & ~\cite{MLthesis,MonoDCell,vlfANN,telco,Qian2019Supervised,uav,csiRNN,wu2019mobile,xu2019efficient,yan2018noise,elbes2019indoor,adege2019mobility,bae2019large,patel2020millimeter,chen2019wifi} &  &  & \\
 \hline
Other & ~\cite{sdr,DNN/KNN,HumanDetection,Timotheatos2017FeatureEA,RelationLearning,hapi,8584443,RamaLocalization,Wang2017WiFiFB,8422182,jaafar2018neural,ge2019hybrid} \cite{felix2016fingerprinting,khatab2017fingerprint,kim2018scalable,wang2019robust,mei2018novel,comiter2017data,comiter2017structured,guo2018accurate,liu2017wicount,adege2018indoor,schmidt2019sdr,malik2019indoor,yi2019neural,sung2019neural,kim2018hybrid,widmaier2019towards,belmonte2019swiblux,xiao2018learning} & ~\cite{8651736,lorawan,10.1145/3321408.3321584,DataAugmentation,Qian2019Supervised} & & ~\cite{lorawan,khatab2017fingerprint,zou2015fast,gu2015online}\\
 \hline
\end{tabularx}
\end{tiny}
\caption{Type of ML model used}
\label{tab:MLType}
\end{table}
% removed cheng2018fingerprint

==> AllTables/LocTypeTbl.tex <==
\begin{table}
\begin{tabularx}{\textwidth} { 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \hline
  & Classification Region & Classification FP & Coordinates \\
 \hline
 Passive & ~\cite{vlfANN} ~\cite{hybloc} & ~\cite{InterpretingCNN} ~\cite{devicefree} ~\cite{gbrbm} ~\cite{8673800} ~\cite{HumanDetection} ~\cite{DCNN} ~\cite{7996460} ~\cite{wu2018accurate} ~\cite{schmidt2019sdr} ~\cite{sanam2018improved} ~\cite{zhao2019accurate} & ~\cite{manifold} ~\cite{FineGrainedSubcarrier} ~\cite{hybloc} ~\cite{schmidt2019sdr} ~\cite{yang2018clustering} ~\cite{chen2019dpr}\\
 \hline
 Active & ~\cite{laperls} ~\cite{8651736} ~\cite{6805641} ~\cite{IndoorOutdoor} ~\cite{8362712} ~\cite{hapi} ~\cite{8008794} ~\cite{yang2012locating} ~\cite{kim2018scalable} ~\cite{kim2018hybrid} ~\cite{secckin2019hierarchical} ~\cite{oussar2011indoor} & ~\cite{FPfusing} ~\cite{NLOS_UWB} ~\cite{OnDevice} ~\cite{lorawan} ~\cite{IndustrialWSN} ~\cite{uav} ~\cite{location_aware} ~\cite{probabilistic_localization} ~\cite{8780770} ~\cite{DNN/KNN} ~\cite{Discriminative} ~\cite{DataAugmentation} ~\cite{8362712} ~\cite{Timotheatos2017FeatureEA} ~\cite{FeatureSelection} ~\cite{RelationLearning} ~\cite{FullBandGSM} ~\cite{hiwl} ~\cite{7064997} ~\cite{JUIndoorLoc} ~\cite{8661625} ~\cite{Wang2017WiFiFB} ~\cite{Chunjing2017WLAN} ~\cite{8422182} ~\cite{cottone2016machine} ~\cite{khatab2017fingerprint} ~\cite{banihashemian2019new} ~\cite{rezgui2017efficient} ~\cite{liu2019hybrid} ~\cite{ahmadi2017exploiting} ~\cite{al2018improved} ~\cite{gu2015online} ~\cite{yan2017hybrid} ~\cite{wang2019indoor} ~\cite{salamah2016enhanced} ~\cite{zhang2019improving} ~\cite{tran2008localization} ~\cite{feng2010location} ~\cite{belmonte2019swiblux} ~\cite{li2019smartloc} ~\cite{livinsa2015localization} & ~\cite{laperls} ~\cite{MLthesis} ~\cite{MassiveMIMO} ~\cite{7743685} ~\cite{MonoDCell} ~\cite{msvr} ~\cite{7938617} ~\cite{6488858} ~\cite{OnDevice} ~\cite{telco} ~\cite{sdr} ~\cite{6805641} ~\cite{wsn_svr} ~\cite{TargetTracking} ~\cite{tdoa} ~\cite{RadioMaps} ~\cite{tlfcma} ~\cite{LowOverhead} ~\cite{magnetic_inertial} ~\cite{patent} ~\cite{dabil} ~\cite{8240410} ~\cite{8108573} ~\cite{10.1145/3321408.3321584} ~\cite{pseudolite} ~\cite{rfid} ~\cite{kmgpr} ~\cite{csiRNN} ~\cite{8765368} ~\cite{Eloc} ~\cite{grof} ~\cite{hapi} ~\cite{mmbp} ~\cite{WeightedAmbientWiFi} ~\cite{eee112} ~\cite{ZhangIndoor} ~\cite{8008794} ~\cite{8584443} ~\cite{8543713} ~\cite{DricotModular} ~\cite{8712551} ~\cite{8931646} ~\cite{LiUnsupervised} ~\cite{AntonioLocalization} ~\cite{RamaLocalization} ~\cite{yang2012locating} ~\cite{8115921} ~\cite{Qian2019Supervised} ~\cite{Zhang2019Wireless} ~\cite{wu2019mobile} ~\cite{feng2019received} ~\cite{jaafar2018neural} ~\cite{pelka2018new} \cite{felix2016fingerprinting} \cite{cheng2018fingerprint} ~\cite{kim2018scalable} ~\cite{yan2018noise} ~\cite{wang2019robust} ~\cite{comiter2017data} ~\cite{nguyen2017performance} ~\cite{musa2019decision} ~\cite{comiter2017structured} ~\cite{zou2015fast} ~\cite{afzal2014localization} ~\cite{figuera2012advanced} ~\cite{guo2018accurate} ~\cite{bi2018adaptive} ~\cite{lee2013new} ~\cite{elbes2019indoor} ~\cite{comiter2018localization} ~\cite{zhang2018heterogeneous} ~\cite{adege2018indoor} ~\cite{adege2019mobility} ~\cite{yan2017hybrid} ~\cite{malik2019indoor} ~\cite{bae2019large} ~\cite{wang2019indoor} ~\cite{yi2019neural} ~\cite{zhang2018enhancement} ~\cite{tewes2019ensemble} ~\cite{kim2018hybrid} ~\cite{xiao2012large} ~\cite{widmaier2019towards} ~\cite{homayounvala2019novel} ~\cite{bhatti2018machine} ~\cite{zhang2019improving} ~\cite{tran2008localization} ~\cite{secckin2019hierarchical} ~\cite{feng2010location} ~\cite{belmonte2019swiblux} ~\cite{li2019smartloc} ~\cite{yang2012locating} ~\cite{xiao2018learning} ~\cite{mahfouz2015kernel} ~\cite{qiu2018walk} ~\cite{yan2015improved} ~\cite{patel2020millimeter}\\
 \hline
 Cooperative &  & ~\cite{alteredAP} ~\cite{wang2007agent} & ~\cite{7504333} ~\cite{mmwave} ~\cite{OpticalCamera}\\
 \hline
\end{tabularx}
 \caption{Type of Classification}
 \end{table}

==> AllTables/LocTypeTbl2.tex <==
\begin{tabularx}{\textwidth} { 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \caption{Type of Classification}
  \label{tab:LocType}
 \hline
  & Classification Region & Classification FP & Coordinates \\
 \hline
 Passive & ~\cite{vlfANN,hybloc} & ~\cite{InterpretingCNN,devicefree,gbrbm,8673800,HumanDetection,DCNN,wu2018accurate,schmidt2019sdr,sanam2018improved,zhao2019accurate} & ~\cite{FineGrainedSubcarrier,hybloc,schmidt2019sdr,yang2018clustering,chen2019dpr}\\
 \hline
 Active & ~\cite{laperls,8651736,6805641,8362712,hapi,8008794,yang2012locating,kim2018scalable,kim2018hybrid,secckin2019hierarchical,oussar2011indoor} & ~\cite{FPfusing,NLOS_UWB,OnDevice,lorawan,IndustrialWSN,uav,location_aware,probabilistic_localization,8780770,DNN/KNN,Discriminative,DataAugmentation,8362712,Timotheatos2017FeatureEA,FeatureSelection,RelationLearning,FullBandGSM,hiwl,7064997,JUIndoorLoc,8661625,Wang2017WiFiFB,Chunjing2017WLAN,8422182,cottone2016machine,khatab2017fingerprint,rezgui2017efficient,liu2019hybrid,ahmadi2017exploiting,gu2015online,yan2017hybrid}  ~\cite{salamah2016enhanced,zhang2019improving,belmonte2019swiblux,li2019smartloc} & ~\cite{laperls,MLthesis,MassiveMIMO,7743685,MonoDCell,7938617}  ~\cite{OnDevice,telco,sdr,6805641,wsn_svr,TargetTracking,tdoa,RadioMaps,tlfcma,LowOverhead,magnetic_inertial,patent,dabil,8240410,8108573,10.1145/3321408.3321584,rfid,kmgpr,csiRNN,8765368,Eloc,grof,hapi,mmbp,WeightedAmbientWiFi,eee112,ZhangIndoor,8008794,8584443,8712551,8931646,LiUnsupervised,AntonioLocalization,RamaLocalization,yang2012locating,8115921,Qian2019Supervised,Zhang2019Wireless,wu2019mobile,feng2019received,jaafar2018neural} \cite{felix2016fingerprinting} \cite{cheng2018fingerprint,kim2018scalable,yan2018noise,wang2019robust,comiter2017data,nguyen2017performance,musa2019decision,comiter2017structured,zou2015fast,figuera2012advanced,guo2018accurate,bi2018adaptive,elbes2019indoor,comiter2018localization,zhang2018heterogeneous,adege2018indoor,adege2019mobility,yan2017hybrid,malik2019indoor,bae2019large,yi2019neural,zhang2018enhancement,tewes2019ensemble,kim2018hybrid,xiao2012large,widmaier2019towards,homayounvala2019novel,bhatti2018machine,zhang2019improving,secckin2019hierarchical,belmonte2019swiblux,li2019smartloc,yang2012locating,xiao2018learning,mahfouz2015kernel,qiu2018walk,patel2020millimeter}\\
 \hline
 Cooperative &  & ~\cite{alteredAP} & ~\cite{7504333,mmwave,OpticalCamera}\\
 \hline
\end{tabularx}
 

==> AllTables/LocTypeTbl3.tex <==
\begin{tabularx}{0.5\textwidth} { 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \caption{Type of Classification}
   \label{tab:LocType}
 \hline
  & Classification Region & Classification FP & Coordinates \\
 \hline
 Passive & ~\cite{vlfANN ,  hybloc} & ~\cite{InterpretingCNN ,  devicefree ,  gbrbm ,  8673800 ,  HumanDetection ,  DCNN ,  wu2018accurate ,  schmidt2019sdr ,  sanam2018improved ,  zhao2019accurate} & ~\cite{FineGrainedSubcarrier ,  hybloc ,  schmidt2019sdr ,  yang2018clustering ,  chen2019dpr}\\
 \hline
 Active & ~\cite{laperls ,  8651736 ,  6805641 ,  8362712 ,  hapi ,  8008794 ,  yang2012locating ,  kim2018scalable ,  kim2018hybrid ,  secckin2019hierarchical ,  oussar2011indoor} & ~\cite{FPfusing ,  NLOS_UWB ,  OnDevice ,  lorawan ,  IndustrialWSN ,  uav ,  location_aware ,  probabilistic_localization ,  8780770 ,  DNN/KNN ,  Discriminative ,  DataAugmentation ,  8362712 ,  Timotheatos2017FeatureEA ,  FeatureSelection ,  RelationLearning ,  FullBandGSM ,  hiwl ,  7064997 ,  JUIndoorLoc ,  8661625 ,  Wang2017WiFiFB ,  Chunjing2017WLAN ,  8422182 ,  cottone2016machine ,  khatab2017fingerprint ,  rezgui2017efficient ,  liu2019hybrid ,  ahmadi2017exploiting ,  gu2015online ,  yan2017hybrid}  ~\cite{salamah2016enhanced ,  zhang2019improving ,  belmonte2019swiblux ,  li2019smartloc} & ~\cite{laperls ,  MLthesis ,  MassiveMIMO ,  7743685 ,  MonoDCell ,  7938617}  ~\cite{OnDevice ,  telco ,  sdr ,  6805641 ,  wsn_svr ,  TargetTracking ,  tdoa ,  RadioMaps ,  tlfcma ,  LowOverhead ,  magnetic_inertial ,  patent ,  dabil ,  8240410 ,  8108573 ,  10.1145/3321408.3321584 ,  rfid ,  kmgpr ,  csiRNN ,  8765368 ,  Eloc ,  grof ,  hapi ,  mmbp ,  WeightedAmbientWiFi ,  eee112 ,  ZhangIndoor ,  8008794 ,  8584443 ,  8712551 ,  8931646 ,  LiUnsupervised ,  AntonioLocalization ,  RamaLocalization ,  yang2012locating ,  8115921 ,  Qian2019Supervised ,  Zhang2019Wireless ,  wu2019mobile ,  feng2019received ,  jaafar2018neural} \cite{felix2016fingerprinting} \cite{cheng2018fingerprint ,  kim2018scalable ,  yan2018noise ,  wang2019robust ,  comiter2017data ,  nguyen2017performance ,  musa2019decision ,  comiter2017structured ,  zou2015fast ,  figuera2012advanced ,  guo2018accurate ,  bi2018adaptive ,  elbes2019indoor ,  comiter2018localization ,  zhang2018heterogeneous ,  adege2018indoor ,  adege2019mobility ,  yan2017hybrid ,  malik2019indoor ,  bae2019large ,  yi2019neural ,  zhang2018enhancement ,  tewes2019ensemble ,  kim2018hybrid ,  xiao2012large ,  widmaier2019towards ,  homayounvala2019novel ,  bhatti2018machine ,  zhang2019improving ,  secckin2019hierarchical ,  belmonte2019swiblux ,  li2019smartloc ,  yang2012locating ,  xiao2018learning ,  mahfouz2015kernel ,  qiu2018walk ,  patel2020millimeter}\\
 \hline
 Cooperative &  & ~\cite{alteredAP} & ~\cite{7504333 ,  mmwave ,  OpticalCamera}\\
 \hline
\end{tabularx}

==> AllTables/SideInfoTbl.tex <==
\begin{tabularx}{\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \caption{Side information}
 \hline
  & Maps & Previous locations & Magnetic Field & Accelerometer \\
 \hline
 Paper & ~\cite{RadioMaps} &  & ~\cite{magnetic_inertial} ~\cite{7064997} ~\cite{IndoorOutdoor} ~\cite{OpticalCamera} ~\cite{Discriminative} ~\cite{8543713} ~\cite{7996460} ~\cite{al2018improved} ~\cite{bae2019large} ~\cite{wang2019indoor} ~\cite{zhou2019smartphone} ~\cite{zhang2019improving} ~\cite{belmonte2019swiblux} ~\cite{qiu2018walk} & ~\cite{6805641} ~\cite{TargetTracking} ~\cite{magnetic_inertial} ~\cite{OpticalCamera} ~\cite{Discriminative} ~\cite{8543713} ~\cite{DricotModular} ~\cite{yang2012locating} ~\cite{zhou2019smartphone} ~\cite{zhang2019improving} ~\cite{belmonte2019swiblux} ~\cite{yang2012locating} ~\cite{qiu2018walk}\\
 \hline
\end{tabularx}

==> AllTables/SideInfoTbl2.tex <==
\begin{tabularx}{\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \caption{Side information}
  \label{tab:SideInfo}
 \hline
  & Maps & Previous locations & Magnetic Field & Accelerometer \\
 \hline
 Paper & ~\cite{RadioMaps} ~\cite{sorour2014joint_47} ~\cite{zhou2017indoor_86} ~\cite{jung2015unsupervised_89} ~\cite{wu2012will_93} & ~\cite{li2019deep_31} ~\cite{zhou2017robust_46} ~\cite{rizk2019solocell_98} ~\cite{zhang2019deeploc_108} & ~\cite{magnetic_inertial} ~\cite{7064997} ~\cite{OpticalCamera} ~\cite{Discriminative} ~\cite{bae2019large} ~\cite{zhang2019improving} ~\cite{belmonte2019swiblux} ~\cite{qiu2018walk} ~\cite{gan2017deep_32} ~\cite{wang2012no_92} ~\cite{zhang2017deeppositioning_106} ~\cite{shao2018indoor_120} & ~\cite{6805641} ~\cite{TargetTracking} ~\cite{magnetic_inertial} ~\cite{OpticalCamera} ~\cite{Discriminative} ~\cite{yang2012locating} ~\cite{zhang2019improving} ~\cite{belmonte2019swiblux} ~\cite{yang2012locating} ~\cite{qiu2018walk} ~\cite{wang2012no_92} ~\cite{wu2012will_93}\\
 \hline
\end{tabularx}

==> AllTables/SideInfoTbl3.tex <==
\begin{tabularx}{.5\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \caption{Side information}
   \label{tab:SideInfo}
 \hline
  & Maps  & Magnetic Field & Accelerometer \\
 \hline
 Paper & ~\cite{RadioMaps,sorour2014joint_47,zhou2017indoor_86,jung2015unsupervised_89,wu2012will_93}   & ~\cite{magnetic_inertial,7064997,OpticalCamera,Discriminative,bae2019large,zhang2019improving,belmonte2019swiblux,qiu2018walk,gan2017deep_32,wang2012no_92,zhang2017deeppositioning_106,shao2018indoor_120} & ~\cite{6805641,TargetTracking,magnetic_inertial,OpticalCamera,Discriminative,yang2012locating,zhang2019improving,belmonte2019swiblux,yang2012locating,qiu2018walk,wang2012no_92,wu2012will_93}\\
 \hline
\end{tabularx}

==> AllTables/StandardTbl.tex <==
\begin{tabularx}{\linewidth} { 
  | >{\raggedright\arraybackslash\hsize=.5\hsize}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=.75\hsize}X |}
 \caption{Wireless Signal used}
 \hline
 %\toprule
  & Wi-Fi & Cellular & BLE & WSN & Other \\
 %\midrule
 \hline
 %\endhead
 RSSI & ~\cite{alteredAP} ~\cite{FPfusing} ~\cite{laperls} ~\cite{MLthesis} ~\cite{7743685} ~\cite{OnDevice} ~\cite{6805641} ~\cite{LowOverhead} ~\cite{magnetic_inertial} ~\cite{patent} ~\cite{OpticalCamera} ~\cite{probabilistic_localization} ~\cite{10.1145/3321408.3321584} ~\cite{kmgpr} ~\cite{DNN/KNN} ~\cite{8765368} ~\cite{Discriminative} ~\cite{8362712} ~\cite{FeatureSelection} ~\cite{hapi} ~\cite{hybloc} ~\cite{7064997} ~\cite{WeightedAmbientWiFi} ~\cite{ZhangIndoor} ~\cite{8008794} ~\cite{8584443} ~\cite{JUIndoorLoc} ~\cite{8931646} ~\cite{yang2012locating} ~\cite{8115921} ~\cite{Qian2019Supervised} ~\cite{8661625} ~\cite{Zhang2019Wireless} ~\cite{Chunjing2017WLAN} ~\cite{8422182} ~\cite{wu2019mobile} ~\cite{feng2019received} ~\cite{zhang2017efficient} ~\cite{ge2019hybrid} \cite{felix2016fingerprinting} \cite{sun2008adaptive} \cite{cheng2018fingerprint} ~\cite{khatab2017fingerprint} ~\cite{kim2018scalable} ~\cite{yan2018noise} ~\cite{wang2019robust} ~\cite{mei2018novel} ~\cite{nguyen2017performance} ~\cite{zou2015fast} ~\cite{rezgui2017efficient} ~\cite{figuera2012advanced} ~\cite{guo2018accurate} ~\cite{bi2018adaptive} ~\cite{elbes2019indoor} ~\cite{liu2019hybrid} ~\cite{adege2018indoor} ~\cite{adege2019mobility} ~\cite{gu2015online} ~\cite{yan2017hybrid} ~\cite{malik2019indoor} ~\cite{zhang2018enhancement} ~\cite{tewes2019ensemble}  ~\cite{kim2018hybrid} ~\cite{xiao2012large} ~\cite{salamah2016enhanced} ~\cite{homayounvala2019novel} ~\cite{zhang2019improving} ~\cite{secckin2019hierarchical} ~\cite{belmonte2019swiblux} ~\cite{li2019smartloc} ~\cite{dashti2016extracting} ~\cite{yang2012locating} ~\cite{xiao2018learning}~\cite{sung2019neural} & ~\cite{MLthesis} ~\cite{MassiveMIMO} ~\cite{MonoDCell} ~\cite{8765368} ~\cite{DataAugmentation} ~\cite{FullBandGSM} ~\cite{wu2019mobile} ~\cite{oussar2011indoor} ~\cite{chen2019dpr} ~\cite{qiu2018walk} & ~\cite{location_aware} ~\cite{dabil} ~\cite{8240410} ~\cite{xu2019efficient} ~\cite{ahmadi2017exploiting} ~\cite{belmonte2019swiblux} & ~\cite{wsn_svr} ~\cite{TargetTracking} ~\cite{LiUnsupervised} ~\cite{RamaLocalization} ~\cite{cottone2016machine} ~\cite{yang2018clustering} ~\cite{li2017measurement} ~\cite{bhatti2018machine} ~\cite{mahfouz2015kernel} & ~\cite{7504333} ~\cite{lorawan} ~\cite{uav} ~\cite{8108573} ~\cite{gbrbm} ~\cite{8780770} ~\cite{rfid} ~\cite{Timotheatos2017FeatureEA} ~\cite{grof} ~\cite{mmbp} ~\cite{hiwl} ~\cite{eee112} ~\cite{DCNN} ~\cite{7313038} ~\cite{xu2019efficient} ~\cite{zhang2018heterogeneous} ~\cite{zhao2019accurate}\\
 \hline
 CSI & ~\cite{InterpretingCNN} ~\cite{MLthesis} ~\cite{devicefree} ~\cite{Eloc} ~\cite{8673800} ~\cite{HumanDetection} ~\cite{RelationLearning} ~\cite{Wang2017WiFiFB} ~\cite{wu2018accurate} ~\cite{schmidt2019sdr} ~\cite{tewes2019ensemble} ~\cite{sanam2018improved} & ~\cite{MLthesis} ~\cite{sdr} ~\cite{liu2017wicount} &  & ~\cite{FineGrainedSubcarrier} & ~\cite{csiRNN} ~\cite{widmaier2019towards}\\
 \hline
 ToA &  ~\cite{ge2019hybrid} &  &  &  & ~\cite{NLOS_UWB} ~\cite{8712551} ~\cite{7313038} ~\cite{zhang2018heterogeneous}\\
 \hline
 Other & ~\cite{FPfusing} ~\cite{tdoa} ~\cite{tlfcma} ~\cite{IndoorOutdoor} ~\cite{AntonioLocalization} ~\cite{comiter2017data} ~\cite{comiter2017structured} & ~\cite{8651736} ~\cite{vlfANN} ~\cite{7938617} ~\cite{telco} ~\cite{tdoa} ~\cite{FullBandGSM} &  & ~\cite{6488858} ~\cite{IndustrialWSN} ~\cite{manifold} ~\cite{DricotModular} ~\cite{7996460} ~\cite{wang2007agent} ~\cite{tran2008localization} ~\cite{livinsa2015localization} ~\cite{yan2015improved} & ~\cite{msvr} ~\cite{RadioMaps} ~\cite{mmwave} ~\cite{8780770} ~\cite{pseudolite} ~\cite{8543713} ~\cite{hossan2018novel} ~\cite{musa2019decision} ~\cite{comiter2018localization} ~\cite{yi2019neural} ~\cite{patel2020millimeter}\\
 \hline
%\bottomrule
\end{tabularx}

==> AllTables/StandardTbl2.tex <==
\begin{tabularx}{\linewidth} { 
  | >{\raggedright\arraybackslash\hsize=.5\hsize}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=.75\hsize}X |}
 \caption{Wireless Signal used}
 \label{tab:Standard}
 \hline
 %\toprule
  & Wi-Fi & Cellular & BLE & WSN & Other \\
 %\midrule
 \hline
 %\endhead
 RSSI & ~\cite{alteredAP} ~\cite{FPfusing} ~\cite{laperls} ~\cite{MLthesis} ~\cite{7743685} ~\cite{OnDevice} ~\cite{6805641} ~\cite{LowOverhead} ~\cite{magnetic_inertial} ~\cite{patent} ~\cite{OpticalCamera} ~\cite{probabilistic_localization} ~\cite{10.1145/3321408.3321584} ~\cite{kmgpr} ~\cite{DNN/KNN} ~\cite{8765368} ~\cite{Discriminative} ~\cite{8362712} ~\cite{FeatureSelection} ~\cite{hapi} ~\cite{hybloc} ~\cite{7064997} ~\cite{WeightedAmbientWiFi} ~\cite{ZhangIndoor} ~\cite{8008794} ~\cite{8584443} ~\cite{JUIndoorLoc} ~\cite{8931646} ~\cite{yang2012locating} ~\cite{8115921} ~\cite{Qian2019Supervised} ~\cite{8661625} ~\cite{Zhang2019Wireless} ~\cite{Chunjing2017WLAN} ~\cite{8422182} ~\cite{wu2019mobile} ~\cite{feng2019received} ~\cite{zhang2017efficient} ~\cite{ge2019hybrid} ~\cite{felix2016fingerprinting} ~\cite{sun2008adaptive} ~\cite{cheng2018fingerprint} ~\cite{khatab2017fingerprint} ~\cite{kim2018scalable} ~\cite{yan2018noise} ~\cite{wang2019robust} ~\cite{mei2018novel} ~\cite{nguyen2017performance} ~\cite{zou2015fast} ~\cite{rezgui2017efficient} ~\cite{figuera2012advanced} ~\cite{guo2018accurate} ~\cite{bi2018adaptive} ~\cite{elbes2019indoor} ~\cite{liu2019hybrid} ~\cite{adege2018indoor} ~\cite{adege2019mobility} ~\cite{gu2015online} ~\cite{yan2017hybrid} ~\cite{malik2019indoor} ~\cite{zhang2018enhancement} ~\cite{tewes2019ensemble} ~\cite{sung2019neural} ~\cite{kim2018hybrid} ~\cite{xiao2012large} ~\cite{salamah2016enhanced} ~\cite{homayounvala2019novel} ~\cite{zhang2019improving} ~\cite{secckin2019hierarchical} ~\cite{belmonte2019swiblux} ~\cite{li2019smartloc} ~\cite{dashti2016extracting} ~\cite{yang2012locating} ~\cite{xiao2018learning} ~\cite{qian2019convolutional_10} ~\cite{ibrahim2018cnn_13} ~\cite{turabieh2019cascaded} ~\cite{akram2018censloc_18} ~\cite{turgut2019deep_27} ~\cite{hsieh2019deep_28} ~\cite{gan2017deep_32} ~\cite{zou2018deep_37} ~\cite{zhang2016deep_38} ~\cite{zhou2017robust_46} ~\cite{sorour2014joint_47} ~\cite{ouyang2011indoor_51} ~\cite{liu2009low_52} ~\cite{gu2015semi_54} ~\cite{pulkkinen2011semi} ~\cite{zhou2017semi_55} ~\cite{wang2020robust_59} ~\cite{aikawa2018wlan_61} ~\cite{abbas2019wideep_63} ~\cite{huang2020widet_64} ~\cite{chen2019wifi_65} ~\cite{ciftler2020federated_70} ~\cite{zhou2017grassma_76} ~\cite{zhou2017indoor_86} ~\cite{chen2018deep_88} ~\cite{jung2015unsupervised_89} ~\cite{wang2012no_92} ~\cite{wu2012will_93} ~\cite{rizk2019device_96} ~\cite{jang2018indoor_99} ~\cite{adege2018applying_102} ~\cite{wang2018deepmap_103} ~\cite{liu2018autloc_104} ~\cite{belmannoubi2019deep_105} ~\cite{zhang2017deeppositioning_106} ~\cite{tarekegn2019applying_107} ~\cite{mittal2018adapting_109} ~\cite{belmannoubi2019stacked_110} ~\cite{adege2018applying_113} ~\cite{soro2019joint_118} ~\cite{song2019novel_119} ~\cite{shao2018indoor_120} ~\cite{zhang2019efficient_122} ~\cite{choi2019unsupervised_123} ~\cite{own2019signal_125} & ~\cite{MLthesis} ~\cite{MassiveMIMO} ~\cite{MonoDCell} ~\cite{8765368} ~\cite{DataAugmentation} ~\cite{FullBandGSM} ~\cite{wu2019mobile} ~\cite{oussar2011indoor} ~\cite{chen2019dpr} ~\cite{qiu2018walk} ~\cite{rizk2018cellindeep_15} ~\cite{zhang2020transfer_49} ~\cite{shokry2018deeploc_50} ~\cite{ray2016localization_94} ~\cite{lee2018dnn_95} ~\cite{rizk2019solocell_98} ~\cite{zhang2019deeploc_108} & ~\cite{location_aware} ~\cite{dabil} ~\cite{8240410} ~\cite{xu2019efficient} ~\cite{ahmadi2017exploiting} ~\cite{belmonte2019swiblux} ~\cite{li2019deep_31} ~\cite{gan2017deep_32} ~\cite{ebuchi2019vehicle_126} & ~\cite{wsn_svr} ~\cite{TargetTracking} ~\cite{LiUnsupervised} ~\cite{RamaLocalization} ~\cite{cottone2016machine} ~\cite{yang2018clustering} ~\cite{li2017measurement} ~\cite{bhatti2018machine} ~\cite{mahfouz2015kernel} ~\cite{chen2011semi_53} ~\cite{ahmadi2015rssi_58} ~\cite{belmannoubi2019stacked_110} & ~\cite{7504333} ~\cite{lorawan} ~\cite{uav} ~\cite{8108573} ~\cite{gbrbm} ~\cite{8780770} ~\cite{rfid} ~\cite{Timotheatos2017FeatureEA} ~\cite{grof} ~\cite{mmbp} ~\cite{hiwl} ~\cite{eee112} ~\cite{DCNN} ~\cite{7313038} ~\cite{xu2019efficient} ~\cite{zhang2018heterogeneous} ~\cite{zhao2019accurate} ~\cite{aikawa2019cnn_16} ~\cite{zheng2016cold_19} ~\cite{janssen2019comparing} ~\cite{njima2019deep_22} ~\cite{wang2016device_39} ~\cite{alhajri2019indoor_74}\\
 \hline
 CSI & ~\cite{InterpretingCNN} ~\cite{MLthesis} ~\cite{devicefree} ~\cite{Eloc} ~\cite{8673800} ~\cite{HumanDetection} ~\cite{RelationLearning} ~\cite{Wang2017WiFiFB} ~\cite{wu2018accurate} ~\cite{schmidt2019sdr} ~\cite{tewes2019ensemble} ~\cite{sanam2018improved} ~\cite{wang2016csi_3} ~\cite{wang2016csi_5} ~\cite{li2018channel_8} ~\cite{wang2017cifi_9} ~\cite{li2019convolutional_12} ~\cite{wang2018deep_23} ~\cite{hsieh2019deep_28} ~\cite{wang2015deepfi_33} ~\cite{yazdanian2018deeppos_34} ~\cite{berruet2018delfin_35} ~\cite{zhou2018device_40} ~\cite{wang2017biloc_43} ~\cite{wu2017passive_44} ~\cite{ghourchian2017real_45} ~\cite{wang2017resloc_56} ~\cite{fukushima2019evaluating_73} ~\cite{sen2012you_91} ~\cite{zhang2019efficient_122} & ~\cite{MLthesis} ~\cite{sdr} ~\cite{liu2017wicount} ~\cite{decurninge2018csi_81} &  & ~\cite{FineGrainedSubcarrier} & ~\cite{csiRNN} ~\cite{widmaier2019towards} ~\cite{van2015machine_1} ~\cite{niitsoo2019deep_2} ~\cite{niitsoo2018convolutional_11} ~\cite{sobehy2019csi_117}\\
 \hline
 ToA &  ~\cite{ge2019hybrid} ~\cite{choi2019unsupervised_69} &  &  &  & ~\cite{NLOS_UWB} ~\cite{8712551} ~\cite{7313038} ~\cite{zhang2018heterogeneous} ~\cite{van2015machine_1} ~\cite{li2017robust_60}\\
 \hline
 Other & ~\cite{FPfusing} ~\cite{tdoa} ~\cite{tlfcma} ~\cite{AntonioLocalization} ~\cite{comiter2017data} ~\cite{comiter2017structured} ~\cite{wu2019csi_7} & ~\cite{8651736} ~\cite{vlfANN} ~\cite{7938617} ~\cite{telco} ~\cite{tdoa} ~\cite{FullBandGSM} ~\cite{butt2020rf_57} &  & ~\cite{IndustrialWSN} & ~\cite{} ~\cite{RadioMaps} ~\cite{mmwave} ~\cite{8780770} ~\cite{musa2019decision} ~\cite{comiter2018localization} ~\cite{yi2019neural} ~\cite{patel2020millimeter} ~\cite{xue2019deeptal_36} ~\cite{bregar2018improving_77}\\
 \hline
%\bottomrule
\end{tabularx}


==> AllTables/StandardTbl3.tex <==
\begin{tabularx}{1\linewidth} { 
  | >{\raggedright\arraybackslash\hsize=.5\hsize}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\raggedleft\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=.75\hsize}X |}
 \caption{Wireless Signal used}
 \label{tab:Standard}
 \hline
 %\toprule
  & Wi-Fi & Cellular & BLE & WSN & Other \\
 %\midrule
 \hline
 %\endhead
 RSSI & ~\cite{alteredAP , FPfusing , laperls , 7743685 , OnDevice , 6805641 , LowOverhead , magnetic_inertial , patent , OpticalCamera , probabilistic_localization , kmgpr , DNN/KNN , 8765368 , Discriminative , 8362712 , FeatureSelection , hapi , hybloc , 7064997 , WeightedAmbientWiFi , ZhangIndoor , 8008794 , 8584443 , JUIndoorLoc , 8931646 , yang2012locating , 8115921 , Qian2019Supervised , 8661625 , Zhang2019Wireless , Chunjing2017WLAN , 8422182 , wu2019mobile , feng2019received , zhang2017efficient , ge2019hybrid , felix2016fingerprinting , sun2008adaptive , cheng2018fingerprint , khatab2017fingerprint , kim2018scalable , yan2018noise , wang2019robust , mei2018novel , nguyen2017performance , zou2015fast , rezgui2017efficient , figuera2012advanced , guo2018accurate , bi2018adaptive , elbes2019indoor , liu2019hybrid , adege2018indoor , adege2019mobility , gu2015online , yan2017hybrid } ~ \cite{ malik2019indoor , zhang2018enhancement , tewes2019ensemble , sung2019neural , kim2018hybrid , xiao2012large , salamah2016enhanced , homayounvala2019novel , zhang2019improving , secckin2019hierarchical , belmonte2019swiblux , li2019smartloc , dashti2016extracting } ~ \cite{ yang2012locating , xiao2018learning , qian2019convolutional_10 , ibrahim2018cnn_13  , akram2018censloc_18 , turgut2019deep_27 , hsieh2019deep_28 , gan2017deep_32 , zou2018deep_37 } ~\cite{zhang2016deep_38 , zhou2017robust_46 , sorour2014joint_47 , ouyang2011indoor_51 , liu2009low_52} ~ \cite{ gu2015semi_54 , pulkkinen2011semi , zhou2017semi_55 , wang2020robust_59} ~\cite{ aikawa2018wlan_61 , abbas2019wideep_63 , huang2020widet_64, XYZXYZ } ~\cite{ ciftler2020federated_70 , zhou2017grassma_76 , zhou2017indoor_86 , chen2018deep_88 , jung2015unsupervised_89 , wang2012no_92 , wu2012will_93 , rizk2019device_96 , jang2018indoor_99}  &   ~\cite{MassiveMIMO , MonoDCell , 8765368 , DataAugmentation ,  FullBandGSM , wu2019mobile ,  oussar2011indoor , chen2019dpr ,  qiu2018walk ,  rizk2018cellindeep_15 ,  zhang2020transfer_49 , shokry2018deeploc_50 ,  ray2016localization_94 ,  lee2018dnn_95 ,  rizk2019solocell_98 , zhang2019deeploc_108} & ~\cite{location_aware ,  dabil ,  8240410 ,  xu2019efficient ,  ahmadi2017exploiting ,  belmonte2019swiblux ,  li2019deep_31 ,  gan2017deep_32 ,  ebuchi2019vehicle_126} & ~\cite{wsn_svr ,  TargetTracking ,  LiUnsupervised ,  RamaLocalization ,  cottone2016machine ,  yang2018clustering ,  li2017measurement ,  bhatti2018machine ,  mahfouz2015kernel ,  chen2011semi_53 ,  ahmadi2015rssi_58 ,  belmannoubi2019stacked_110 } & ~\cite{7504333 ,  lorawan ,  uav ,  8108573 ,  gbrbm ,  8780770 ,  rfid ,  Timotheatos2017FeatureEA ,  grof ,  mmbp ,  hiwl ,  eee112 ,  DCNN ,  7313038 ,  xu2019efficient ,  zhang2018heterogeneous ,  zhao2019accurate ,  aikawa2019cnn_16 ,  zheng2016cold_19 ,    njima2019deep_22 ,  wang2016device_39 ,  alhajri2019indoor_74}\\
 \hline
 CSI & ~\cite{InterpretingCNN,devicefree ,  Eloc ,  8673800 ,  HumanDetection ,  RelationLearning ,  Wang2017WiFiFB ,  wu2018accurate ,  schmidt2019sdr ,  tewes2019ensemble ,  sanam2018improved ,  wang2016csi_3 ,  wang2016csi_5 ,  li2018channel_8 ,  wang2017cifi_9 ,  li2019convolutional_12 ,  wang2018deep_23 ,  hsieh2019deep_28 ,  wang2015deepfi_33 ,  yazdanian2018deeppos_34 ,  berruet2018delfin_35 ,  zhou2018device_40}  ~\cite{wu2017passive_44 ,  ghourchian2017real_45 ,  wang2017resloc_56 ,  fukushima2019evaluating_73 ,  sen2012you_91 ,  zhang2019efficient_122} &  \cite{sdr ,  liu2017wicount ,  decurninge2018csi_81} &  & ~\cite{FineGrainedSubcarrier} & ~\cite{csiRNN ,  widmaier2019towards ,  van2015machine_1 ,  niitsoo2019deep_2 ,  niitsoo2018convolutional_11 ,  sobehy2019csi_117}\\
 \hline
 ToA &  ~\cite{ge2019hybrid ,  choi2019unsupervised_69} &  &  &  & ~\cite{NLOS_UWB ,  8712551 ,  7313038 ,  zhang2018heterogeneous ,  van2015machine_1 ,  li2017robust_60}\\
 \hline
 Other & ~\cite{FPfusing ,  tdoa ,  tlfcma ,  AntonioLocalization ,  comiter2017data ,  comiter2017structured ,  wu2019csi_7} & ~\cite{8651736 ,  vlfANN ,  7938617 ,  telco ,  tdoa ,  FullBandGSM ,  butt2020rf_57} &  & ~\cite{IndustrialWSN} & ~\cite{    RadioMaps ,  mmwave ,  8780770 ,  musa2019decision ,  comiter2018localization ,  yi2019neural ,  patel2020millimeter ,  xue2019deeptal_36 ,  bregar2018improving_77}\\
 \hline
%\bottomrule
\end{tabularx}

==> AllTables/StandardTbl4.tex <==
\begin{table}
\begin{tiny}
\begin{tabularx}{0.95\linewidth} { 
  | >{\raggedright\arraybackslash\hsize=.75\hsize}X 
  | >{\centering\arraybackslash\hsize=1.05\hsize}X 
  | >{\raggedleft\arraybackslash\hsize=1.05\hsize}X 
  | >{\raggedleft\arraybackslash\hsize=1.05\hsize}X 
  | >{\centering\arraybackslash\hsize=1.05\hsize}X 
  | >{\centering\arraybackslash\hsize=1.05\hsize}X |}
 \hline
 %\toprule
  & Wi-Fi & Cellular & BLE & WSN & Other \\
 %\midrule
 \hline
 %\endhead
 RSSI & ~\cite{alteredAP , FPfusing , laperls , 7743685 , OnDevice , 6805641 , LowOverhead , magnetic_inertial , patent , OpticalCamera , probabilistic_localization , kmgpr , DNN/KNN , 8765368 , Discriminative , 8362712 , FeatureSelection , hapi , hybloc , 7064997 , WeightedAmbientWiFi , ZhangIndoor , 8008794 , 8584443 , JUIndoorLoc , 8931646 , yang2012locating , 8115921 , Qian2019Supervised , 8661625 , Zhang2019Wireless , Chunjing2017WLAN , 8422182 , wu2019mobile , feng2019received , zhang2017efficient , ge2019hybrid , felix2016fingerprinting , sun2008adaptive  , khatab2017fingerprint , kim2018scalable , yan2018noise , wang2019robust , mei2018novel , nguyen2017performance , zou2015fast , rezgui2017efficient , figuera2012advanced , guo2018accurate , bi2018adaptive , elbes2019indoor , liu2019hybrid , adege2018indoor , adege2019mobility , gu2015online , yan2017hybrid , malik2019indoor , zhang2018enhancement , tewes2019ensemble , sung2019neural , kim2018hybrid , xiao2012large , salamah2016enhanced , homayounvala2019novel , zhang2019improving , secckin2019hierarchical , belmonte2019swiblux , li2019smartloc , dashti2016extracting , yang2012locating , xiao2018learning , qian2019convolutional_10 , ibrahim2018cnn_13  , akram2018censloc_18 , turgut2019deep_27 , hsieh2019deep_28 , gan2017deep_32 , zou2018deep_37 , zhang2016deep_38 , zhou2017robust_46 , sorour2014joint_47 , ouyang2011indoor_51 , liu2009low_52, gu2015semi_54 , pulkkinen2011semi , zhou2017semi_55 , wang2020robust_59, aikawa2018wlan_61 , abbas2019wideep_63 , huang2020widet_64, chen2019wifi } ~\cite{ ciftler2020federated_70 , zhou2017grassma_76 , zhou2017indoor_86 , chen2018deep_88 , jung2015unsupervised_89 , wang2012no_92 , wu2012will_93 , rizk2019device_96 , jang2018indoor_99}  
 
 &   ~\cite{MassiveMIMO , MonoDCell , 8765368 , DataAugmentation ,  FullBandGSM , wu2019mobile ,  oussar2011indoor , chen2019dpr ,  qiu2018walk ,  rizk2018cellindeep_15 ,  zhang2020transfer_49 , shokry2018deeploc_50 ,  ray2016localization_94 ,  lee2018dnn_95 ,  rizk2019solocell_98 , zhang2019deeploc_108} 
 
 & ~\cite{location_aware ,  dabil ,  8240410 ,  xu2019efficient ,  ahmadi2017exploiting ,  belmonte2019swiblux ,  li2019deep_31 ,  gan2017deep_32 ,  ebuchi2019vehicle_126, peng2016iterative}
 
 & ~\cite{wsn_svr ,  TargetTracking ,  LiUnsupervised ,  RamaLocalization ,  cottone2016machine ,  yang2018clustering ,  li2017measurement ,  bhatti2018machine ,  mahfouz2015kernel ,  chen2011semi_53 ,  ahmadi2015rssi_58 ,  belmannoubi2019stacked_110 , nguyen2005kernel} 
 
 & ~\cite{7504333 ,  lorawan ,  uav ,  8108573 ,  gbrbm ,  8780770 ,  rfid ,  Timotheatos2017FeatureEA ,  grof  ,  hiwl ,  eee112 ,  DCNN ,  7313038 ,  xu2019efficient ,  zhang2018heterogeneous ,  zhao2019accurate ,  aikawa2019cnn_16 ,  zheng2016cold_19 ,    njima2019deep_22 ,  wang2016device_39 ,  alhajri2019indoor_74}\\
 %------------------------------------------------------------------
 \hline
 CSI & ~\cite{InterpretingCNN,devicefree ,  Eloc ,  8673800 ,  HumanDetection ,  RelationLearning ,  Wang2017WiFiFB ,  wu2018accurate ,  schmidt2019sdr ,  tewes2019ensemble ,  sanam2018improved ,  wang2016csi_3 ,  wang2016csi_5 ,  li2018channel_8 ,  wang2017cifi_9 ,  li2019convolutional_12 ,  wang2018deep_23 ,  hsieh2019deep_28 ,  wang2015deepfi_33 ,  yazdanian2018deeppos_34 ,  berruet2018delfin_35 ,  zhou2018device_40, wu2017passive_44 ,  ghourchian2017real_45 ,  wang2017resloc_56 ,  fukushima2019evaluating_73 ,  sen2012you_91 ,  zhang2019efficient_122} &  \cite{sdr ,  liu2017wicount ,  decurninge2018csi_81} &  & ~\cite{FineGrainedSubcarrier} & ~\cite{csiRNN ,  widmaier2019towards ,  van2015machine_1 ,  niitsoo2019deep_2 ,  niitsoo2018convolutional_11 ,  sobehy2019csi_117}\\
  %------------------------------------------------------------------

 \hline
 ToA &  ~\cite{ge2019hybrid ,  choi2019unsupervised_69} &  &  &  & ~\cite{NLOS_UWB ,  8712551 ,  7313038 ,  zhang2018heterogeneous ,  van2015machine_1 ,  li2017robust_60}\\
 
 \hline
 Other & ~\cite{roshanaei2009dynamic,FPfusing ,  tdoa ,  tlfcma ,  AntonioLocalization ,  comiter2017data ,  comiter2017structured ,  wu2019csi_7}
 & ~\cite{8651736 ,  vlfANN ,  7938617 ,  telco ,  tdoa ,  FullBandGSM ,  butt2020rf_57} &  & ~\cite{IndustrialWSN} 
 & ~\cite{    RadioMaps ,  mmwave ,  8780770 ,  musa2019decision ,  comiter2018localization ,  yi2019neural ,  patel2020millimeter ,  xue2019deeptal_36 ,  bregar2018improving_77}\\
 \hline
%\bottomrule
\end{tabularx}
\end{tiny}
\caption{Wireless Signal used}
\label{tab:Standard}
\end{table}
% removed cheng2018fingerprint

==> AllTables/WirelessTechTbl.tex <==
\begin{tabularx}{\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \caption{Technology}
 \hline
  & Papers \\
 \hline
 OFDM & ~\cite{uav}\\
 \hline
 MIMO & \\
 \hline
 Massive MIMO & ~\cite{MassiveMIMO} ~\cite{widmaier2019towards}\\
 \hline
 Distributed MIMO & ~\cite{MassiveMIMO}\\
 \hline
 UWB & ~\cite{NLOS_UWB} ~\cite{IndustrialWSN} ~\cite{8712551} ~\cite{7313038} ~\cite{musa2019decision} ~\cite{savic2014kernel}\\
 \hline
\end{tabularx}

==> AllTables/WirelessTechTbl2.tex <==
\begin{tabularx}{\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \caption{Technology}
 \label{tab:Technology}
 \hline
  & Papers \\
 \hline
 OFDM & ~\cite{uav,wang2016csi_5,wu2019csi_7,li2018channel_8,wang2017cifi_9,li2019convolutional_12,hsieh2019deep_28,wang2015deepfi_33,berruet2018delfin_35,wang2017biloc_43,wu2017passive_44,ghourchian2017real_45,wang2017resloc_56,butt2020rf_57,fukushima2019evaluating_73,wu2019learning_78,sun2019fingerprint_79,vieira2017deep_80,decurninge2018csi_81,arnold2018deep_82,sun2018single_90,sobehy2019csi_117,lei2019siamese_130}\\
 \hline
 MIMO & ~\cite{niitsoo2019deep_2} \cite{wang2016csi_3,wang2016csi_5,li2018channel_8,wang2017cifi_9,li2019convolutional_12,wang2018deep_23,hsieh2019deep_28,wang2015deepfi_33,berruet2018delfin_35,wang2017biloc_43,wu2017passive_44,ghourchian2017real_45,wang2017resloc_56,butt2020rf_57,fukushima2019evaluating_73,arnold2018deep_82,chen2018multipath_111,sobehy2019csi_117,zhang2019efficient_122,lei2019siamese_130,jing2019learning_131}\\
 \hline
 Massive MIMO & ~\cite{MassiveMIMO,widmaier2019towards,prasad2018machine_62,wu2019learning_78,sun2019fingerprint_79,vieira2017deep_80,decurninge2018csi_81,wang2019fast_83,prasad2017numerical_84,sun2018single_90,de2019csi_121}\\
 \hline
 Distributed MIMO & ~\cite{MassiveMIMO,prasad2018machine_62,prasad2017numerical_84,pirzadeh2019machine_87}\\
 \hline
 UWB & ~\cite{NLOS_UWB,IndustrialWSN,8712551,7313038,musa2019decision,van2015machine_1,xue2019deeptal_36,kram2019uwb_68,krishnan2018improving_71}\\
 \hline
\end{tabularx}

==> AllTables/WirelessTechTbl3.tex <==
\vspace{10 mm}
\begin{tabularx}{0.5\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X |}
 \caption{Technology}
 \label{tab:Technology}
 \hline
  & Papers \\
 \hline
  OFDM & ~\cite{uav,wang2016csi_5,wu2019csi_7,li2018channel_8,wang2017cifi_9,li2019convolutional_12,hsieh2019deep_28,wang2015deepfi_33,berruet2018delfin_35, wu2017passive_44,ghourchian2017real_45,wang2017resloc_56,butt2020rf_57,fukushima2019evaluating_73,wu2019learning_78,sun2019fingerprint_79,vieira2017deep_80,decurninge2018csi_81,arnold2018deep_82,sun2018single_90,sobehy2019csi_117,lei2019siamese_130}\\
 \hline
 MIMO & ~\cite{niitsoo2019deep_2} \cite{wang2016csi_3,wang2016csi_5,li2018channel_8,wang2017cifi_9,li2019convolutional_12,wang2018deep_23,hsieh2019deep_28,wang2015deepfi_33,berruet2018delfin_35, wu2017passive_44,ghourchian2017real_45,wang2017resloc_56,butt2020rf_57,fukushima2019evaluating_73,arnold2018deep_82,chen2018multipath_111,sobehy2019csi_117,zhang2019efficient_122,lei2019siamese_130,jing2019learning_131}\\
 \hline
 Massive MIMO & ~\cite{MassiveMIMO,widmaier2019towards,prasad2018machine_62,wu2019learning_78,sun2019fingerprint_79,vieira2017deep_80,decurninge2018csi_81,wang2019fast_83,prasad2017numerical_84,sun2018single_90,de2019csi_121}\\
 \hline
 Distributed MIMO & ~\cite{MassiveMIMO,prasad2018machine_62,prasad2017numerical_84,pirzadeh2019machine_87}\\
 \hline
 UWB & ~\cite{NLOS_UWB,IndustrialWSN,8712551,7313038,musa2019decision,van2015machine_1,xue2019deeptal_36,kram2019uwb_68,krishnan2018improving_71}\\
 \hline
\end{tabularx}

==> DeepTemp.tex <==
103	Wang, Xiangyu, et al. "DeepMap: Deep Gaussian Process for indoor radio map construction and location estimation." 
	IEEE Global Communications Conference (GLOBECOM). IEEE, 2018.	For RSS fingerprinting based localization : employs deep Gaussian process for constructing received signal
strength (RSS) radio maps and a Bayesian algorithm for online localization	two-layer deep Gaussian process model
to capture the relationship between the RSS space and the location space and provide an offline Bayesian training method
to determine model parameters	RSS from APs	Gaussian process is a kernel based Bayesian model, a Dell laptop or a smartphone can be used as a mobile device. We use Gaussian process for indoor localization
as a benchmark, All the RSS data is collected from 433 APs,	The results
show that DeepMap achieves higher localization accuracy
with moderate training data comparing to the Gaussian
process approach	1,g
Dep
GP

	S_O
Deep GP Bayesian algorithm for online localization	RSSI						wifi		Meas.		wang2018deepmap_103

==> Other.tex <==
       %% Use several solutions
        \item Full-Band GSM Fingerprints for Indoor Localization Using a Machine Learning Approach~\cite{FullBandGSM}
    \begin{itemize}
        \item \textbf{Description:} This paper is the ﬁrst study to use ﬁngerprints containing all GSM carriers, as well as the ﬁrst to suggest that GSM can be useful for localization of very high performance. First Principal Component Analysis (PCA) is used for dimensionality reduction, and then the fingerprints are input to a Machine Learning model for classification of user location.
        \item \textbf{Training:} supervised
        \item \textbf{Localization type:} classification
        \item \textbf{Wireless Signal:} Received Signal Strength (RSS) and Base Station Identity Code (BSIC)
        \item \textbf{Localization side:} centralized 
        \item \textbf{Goal} active 
        \item \textbf{Environment type:} Indoor 
        \item \textbf{Side information:} entire set contains 498 GSM carriers out of which 10 were found to contain no energy and were removed from the study.  
        \item \textbf{Model:} K-Nearest Neighbor (K-NN), Support Vector Machine (SVM), Multilayer Perceptron (MLP), and Gaussian Process (GP) classiﬁers. 
        \item \textbf{Technology:} Cellular (GSM). 
        \item \textbf{Antenna:} Not mentioned.
        \item \textbf{Base station (access point) data:} multiple
        \item \textbf{Test data:} The TEMS trace mobile system.
        \item \textbf{ML framework:} The Spider SVM package
        \item \textbf{Error values:} The linear Support Vector Machine provides mean room classiﬁcation accuracy of almost 98\% when all GSM carriers are used. 
        \item \textbf{Training Data Point Number:} cross-validation with ten independent randomly selected splits, each one containing 169 training examples and 72 validation examples.
        \item \textbf{Training Point Resolution:} Not mentioned. 
        \item \textbf{Publication year and number of citations:}  2010 and 25 citations.
        \item \textbf{Did they use open data set?:} No
        \item \textbf{Is their source code available online?:} No 
    \end{itemize}
    
    %% Updating Solution:
        \item An Eﬃcient Radio Map Updating Algorithm based on K-Means and Gaussian Process Regression~\cite{kmgpr}
    \begin{itemize}
        \item \textbf{Description:} In this paper, an eﬃcient radio map updating algorithm is proposed based on K-Means and Gaussian Process Regression (KMGPR) to reduce the workload in updating a ﬁngerprint-based indoor localisation radio map. First, a GPR predictive model is built from the RSS values based on a Gaussian mean function. Then the radio is updated map with online K-Means clustering.  
        \item \textbf{Training:} supervised
        \item \textbf{Localization type:} coordinates
        \item \textbf{Wireless Signal:} RSS
        \item \textbf{Localization side:} centralized  
        \item \textbf{Goal} active 
        \item \textbf{Environment type:} Indoor
        \item \textbf{Side information:} None
        \item \textbf{Model:}  K-Means and Gaussian Process Regression (KMGPR)
        \item \textbf{Technology:} Wi-Fi 
        \item \textbf{Antenna:} Not mentioned.
        \item \textbf{Base station (access point) data:} 9 APs in the first scenario, 6 APs in the second scenario.
        \item \textbf{Test data:}  Smartphone (Samsung Nexus S)
        \item \textbf{ML framework:} Not mentioned.
        \item \textbf{Error values:} In the first scenario, for 100 RPs, average localization errors are 2.475m for zero mean, 2.376 for constant mean, 2.639 for linear mean and 2.078m for Gaussian mean. In the second scenario, for 60 RPs, average localization errors are 2.381m for zero mean, 2.264 for constant mean, 2.915 for linear mean and 1.984 for Gaussian mean.
        \item \textbf{Training Data Point Number:} For first scenario, 105 reference points (RPs), 20 fingerprints at each point. Total 2100 fingerprints for training. 96 points for testing. For second scenario, 65 RPs, 20 RSS samples from each point. Total 1300 fingerprints for training. 34 locations for testing.
        \item \textbf{Training Point Resolution:} Not mentioned.
        \item \textbf{Publication year and number of citations:} 2018 and 3 citations.
        \item \textbf{Did they use open data set?:} In the ﬁrst scenario, the experimental dataset introduced by Laoudias et al.~\cite{Laoudias2013devices} was used.
        \item \textbf{Is their source code available online?:} No
    \end{itemize}
    

==> OtherSolutions.tex <==
    
